Study of potential self-annihilation signal from dark matter particles in some prospective astrophysical dark matter sources

With the growing interest in indirect detection for dark matter signature, the thesis aims to investigate the signal originating from the self-annihilation of dark matter candidates. The methods for targeting the dark matter signal are two-fold, on one hand, we explore the gamma rays resulting from dark matter particles. On the other hand, we focus on complementary radio properties.

==> chapters/chapter11.tex <==
\section{Reply to Examiner's Comment}
%\Date

\hrulefill \\

\section{Authors' Reply}
Author of the thesis entitled \textbf{``Study Of Potential Self-Annihilation Signal From Dark Matter Particles In Some Prospective Astrophysical Dark Matter Sources"} thank the examiner very much for pointing out few important and valid points. All the responses are given below.

\subsection{Questions to be clarified in the text/during viva-voce.}
\begin{enumerate}
\item Referee's Comments: \\
\noindent Discuss the bounds/exclusions on mass of non-baryonic DM from previous searches.\\
 
\textbf{Author's response :} \\  
\noindent I discussed the possible bounds on DM mass obtaining from previous searches in the conclusion section of Chapter 6.\\

\item Referee's Comments: \\
\noindent \textbf{(Section 3.2)} Table 3.1 mentions that the energy resolution is $<$ 15$\%$ at $>$ 100 MeV.
How the energy resolution of the Fermi-LAT depends on the energy of the incident photon?
What are the factors that affect the energy resolution of the detector? How is it possible to
have a good energy resolution, when for a high energy photon ($>$100 GeV), ``most of the
shower fall outside the active region of CAL''?\\

\textbf{Author's response :} \\  
\noindent The energy resolution of the Fermi-LAT strongly depends on the energy of the incident photons. Between 1 GeV and 100 GeV (which is the best region for spectral analysis), the energy resolution of Fermi-LAT is $<10\%$ whereas at 100 MeV it is around $20\%$ at MeV. 
At low energy, the spacecraft orbits with high particle backgrounds and that increases the activity of LAT as well as reduce the photon selection efficiency. At high energy, the limitations of the LAT approach are mostly due to the small statistics available.
In Pass 8 the Fermi-LAT collaboration team introduced a clustering stage, which proved to be very effective to improve the energy resolution at high energy.\\

\item Referee's Comments: \\
\noindent \textbf{(Section 6.4)} In Fig. 6.2(a), with nine years of Fermi-LAT data, 
for 100$\%$ $b\bar{b}$ channel the TS value peaks at $m_{DM}$ = 14 GeV, while for 100$\%$ $\tau^{+} + \tau^{-}$ it peaks at $m_{DM}$ = 4 GeV [20]. Have you checked, if the peak value of TS varies (14 GeV for $b\bar{b}$ and 4 GeV for $\tau^{+} + \tau^{-}$) with the amount of data used in analysis. Figure 6.2(a) seems to indicate that the
position of the peak value for TS is changing with the amount of data analysed.\\
 
\textbf{Author's response :} \\  
\noindent Yes, we checked whether the peak TS value varies with periods of data and found that the peak value is more or less constant.\\
 
\item Referee's Comments: \\
\noindent \textbf{(Figure 6.3)} Comment on how the `error bars' in the figure have been assigned – statistical or statistical+
systematic. The error bars are large in the region of interest (in the right plot). The (apparent) excess is over a rather large range of energy.\\
 
\textbf{Author's response :} \\  
\noindent At lower energy, the large `error bars' are mainly caused by the systematic of the instrument.\\

\item Referee's Comments: \\
\noindent \textbf{(Section 6.4.1, P69)}
There were many earlier studies that already analyzed Tuc-II with six or seven years of Fermi-LAT data [212–215]. But in our analysis, we have studied Tuc-II with nine years of Fermi-LAT data and thus the increase in TS peak values possibly originate from the larger dataset [20]. Hence, such an increase in $\gamma$-ray excess with increasing the time period of $\gamma$-ray excess with increasing the time period of analysis seems to encourage the indirect detection of DM annihilation signal [20].

If possible, add results from previous analyses in table 6.5 or figure 6.2. Add a comment
in the text too.\\
 
\textbf{Author's response :} \\  
\noindent I added few lines in Chapter 6.\\

\item Referee's Comments: \\
\noindent \textbf{(P71)} How p-value is calculated should be defined in chapter 4 or in the annexure.\\
 
\textbf{Author's response :} \\  
\noindent I described the p-value calculation in Chapter 4.\\

\item Referee's Comments: \\
\noindent What improvements in the observations (detector, data analysis, etc) can make your results more robust and put more stringent limits?\\
 
\textbf{Author's response :} \\  
\noindent There are several ways to improve our results. The most three important factors are 1) periods of data, 2) improving the sensitivity of the detector, 3) improving the energy and angular resolutions.\\

\item Referee's Comments: \\
\noindent \textbf{(P83)} What are the future experiments that can investigate the excess seen in Tuc-II?
Discuss the features of the future experiments which can help resolve the issue.\\
 
\textbf{Author's response :} \\  
\noindent  The Cherenkov Telescope Array (CTA) would be the most crucial detector to investigate the excess seen in Tuc-II. I discussed this in Chapters 7 and 8.\\

\item Referee's Comments: \\
\noindent Table 7.8 shows that J values calculated using NFW, ISO and BURKERT vary widely for
UGC 3371, etc. But, Table 8.2 shows that the J values obtained from them are close for
Aquarius II, etc. Please explain the difference.\\
 
\textbf{Author's response :} \\  
\noindent The value of the J-factor could be very different for each source. We can only compare them for alike sources.\\
 
\end{enumerate}
\hrulefill \\
\subsection{General Editorial Comments}
\begin{enumerate}
\item   Referee's comment: \\
\noindent References should appear in sequence. The first reference that appears in the text is
[25] whereas reference [1] comes after [39]. \\

\textbf{Author's response :} \\    
    
\noindent I corrected the reference sequence.\\

\item   Referee's comment: \\
    \textbf{Use of capital letters in the section titles should be uniform. See the disparity below.}\\
\noindent 1.3 Observational Evidence of Dark Matter.\\
\noindent 1.4.2 Weakly interacting massive particles.\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I corrected this mistake.\\

\item   Referee's comment: \\
\noindent Avoid using ‘artist’s rendition’ type figures/diagrams, replace if possible. \\

\textbf{Author's response :} \\    
    
\noindent I modified the images.\\  

\item   Referee's comment: \\
\noindent Full form and meaning of terms like TSTART (MET), TSTOP (MET) be mentioned.\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I made the changes.\\

\end{enumerate}
\hrulefill \\
\subsection{Specific Editorial Comments}
\begin{enumerate}
\item Referee's comment : \\
\noindent \textbf{Abstract}\\
\noindent \textbf{P5}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the sentence in Abstract (P5).\\

\item Referee's comment : \\
\noindent \textbf{Section 1.1}\\
\noindent \textbf{P1}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the sentence in section 1.1 (P1).\\

\item Referee's comment : \\
\noindent \textbf{P2}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the paragraph (P2).\\

\item Referee's comment : \\
\noindent \textbf{P3 first para}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the paragraph (P3 first para).\\

\item Referee's comment: \\
\noindent `Unfortunately, we are yet to detect this strange material in the laboratory.' Remove this sentence as the same is stated in the next.\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I removed the sentence.\\

\item Referee's comment : \\
\noindent \textbf{Section 1.2}\\
\noindent \textbf{P3}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the sentence in section 1.2 (P3).\\
 

\item   Referee's comment : \\
\noindent \textbf{Section 1.2:}:\\
\noindent \textbf{P4}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the sentences in section 2.1 (P4).\\

\item   Referee's comment : \\
\noindent \textbf{P5}

\textbf{Author's response :} \\    
    
\noindent I added the abbreviation for HI.\\
\noindent Like the referee’s suggestion, I modified the sentences in section 1.2 (P4).\\

\item   Referee's comment : \\
\noindent \textbf{Section 1.3}

\textbf{Author's response :} \\    
    
\noindent I followed all the referee's suggestions and modified the Section 1.3 accordingly.

\item   Referee's comment : \\
\noindent \textbf{P6}

\textbf{Author's response :} \\    
    
\noindent  Like the referee’s suggestion, I modified the sentences in P6.\\

\item   Referee's comment : \\
\noindent \textbf{P7}

\textbf{Author's response :} \\    
    
\noindent  I followed all the suggestions that the referee suggested for P7.\\

\item   Referee's comment : \\
\noindent \textbf{P8}

\textbf{Author's response :} \\    
    
\noindent  I replaced the figure 1.3.\\

\item   Referee's comment : \\
\noindent \textbf{Section 1.4}
\noindent \textbf{P9}

\textbf{Author's response :} \\    
    
\noindent  I followed all the referee's suggestions and incorporated the changes in P9 accordingly.\\

\item   Referee's comment : \\
\noindent \textbf{P10}

\textbf{Author's response :} \\    
    
\noindent  I followed all the referee's suggestions and incorporated the changes in P10 accordingly.\\

\item   Referee's comment : \\
\noindent \textbf{P11}

\textbf{Author's response :} \\    
    
\noindent  I followed all the referee's suggestions and incorporated the changes in P11 accordingly.\\

\item   Referee's comment : \\
\noindent \textbf{P12}\\

\textbf{Author's response :} \\    
    
\noindent  I followed all the suggestions that the referee suggested for P12.\\

\item   Referee's comment : \\
\noindent \textbf{Section 1.5}\\
\noindent \textbf{P12}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for Section 1.5 (P12).\\

\item   Referee's comment : \\
\noindent \textbf{Section P13}\\
\noindent \textbf{Figure 1.5 – make it bigger.}\\

\textbf{Author's response :} \\    
    
\noindent I increased the size of figure 1.5.\\

\item   Referee's comment : \\
\noindent \textbf{P14}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for P14.\\

\item   Referee's comment : \\
\noindent \textbf{Section 1.6}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the sentences in section 1.6.\\

\item   Referee's comment : \\
\noindent \textbf{Section 1.6.1}\\
\noindent \textbf{P16}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I incorporated the changes in section 1.6.1 (P16).\\

\item   Referee's comment : \\
\noindent \textbf{Section 1.6.3}\\
\noindent \textbf{P19}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for Section 1.6.3 (P19).\\

\item   Referee's comment : \\
\noindent \textbf{Section 2.1}\\
\noindent \textbf{dwarf spheroidal galaxies (dSphs) – this abbreviation is mentioned 3 times in this chapter!}\\

\textbf{Author's response :} \\    
    
\noindent I made the necessary changes.\\

\item   Referee's comment : \\
\noindent \textbf{P21}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for P21.\\

\item   Referee's comment : \\
\noindent \textbf{P22}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for P22.\\

\item   Referee's comment : \\
\noindent \textbf{Section 2.1}
\noindent \textbf{P23, P24}\\
\noindent \textbf{Explain the symbols properly.}

\textbf{Author's response :} \\    
    
\noindent In the corrected copy, I used the different symbols for each density profile and explained them properly.\\

\item   Referee's comment : \\
\noindent \textbf{P25, P26}\\
\noindent \textbf{DMFIT, DMFit – please make it uniform}\\
\noindent \textbf{DMFIT, Dark-SUSY, Pythia - references given multipple times - please remove.}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I used the uniform abbreviation. I also removed the repetitive references.\\

\item   Referee's comment : \\
\noindent \textbf{2.3.2}
\noindent \textbf{P26}\\
\noindent \textbf{Include the definition of $\theta_{min}$ and its numerical value used.}\\
\noindent \textbf{Include the definition of tidal radius $R_{t}$ and its numerical value used.}\\
\noindent \textbf{What is d in equation 2.8?}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I added the definition of $\theta_{min}$, $R_{t}$ and d in P26.\\

\item   Referee's comment : \\
\noindent \textbf{Section 2.3.4}
\noindent \textbf{P28}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for P28.\\

\item   Referee's comment : \\
\noindent \textbf{Section 2.4}
\noindent \textbf{P28-P29}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for Section 2.4.\\

\item   Referee's comment : \\
\noindent \textbf{P29}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I incorporated all the changes in P29.\\


\item   Referee's comment : \\
\noindent \textbf{P32}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I incorporated all the changes in P32.\\

\item   Referee's comment : \\
\noindent \textbf{Section 3.1}
\noindent \textbf{P36}\\

\textbf{Author's response :} \\    
    
\noindent I followed all the suggestions that the referee suggested for Section 3.1.\\

\item   Referee's comment : \\
\noindent \textbf{Section 3.2.3}
\noindent \textbf{P38}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I made the necessary changes.\\

\item  Referee's comment : \\
\noindent \textbf{Section 3.2.3.2}
\noindent \textbf{P40}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I incorporated all the changes in Section 3.2.3.2.\\

\item   Referee's comment : \\
\noindent \textbf{Section 3.2.5}
\noindent \textbf{P42}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I incorporated all the changes in Section 3.2.5.\\

\item   Referee's comment : \\
\noindent \textbf{P42-P43}\\
\noindent \textbf{Give reference for `PASS 8’.}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I added the reference for `PASS 8'.\\

\item   Referee's comment : \\
\noindent \textbf{Section 4.2.}
\noindent \textbf{P45}\\

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I incorporated all the changes in Section 4.2.\\

\item   Referee's comment : \\
\noindent \textbf{Section 5.2}
\noindent \textbf{P52}\\
\noindent \textbf{Explain `event class' and `event type', particularly `event class 128' and `event type 3'.}

\textbf{Author's response :} \\    
    
\noindent I explained the term `event class’ and `event type’ in Section 5.2.\\

\item   Referee's comment: \\
\noindent \textbf{Section 5.2}
\noindent \textbf{P52; Figure 5.1}\\
\noindent \textbf{The lines in the upper plot should be adequately explained
using legends in the figure itself as well as in the caption and the text. See figure 5.2 for example.}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I made the necessary changes in the caption of Figure 5.2 and also added few lines in Section 5.2.\\


\item   Referee's comment : \\
\noindent \textbf{Section 6.1}
\noindent \textbf{P63}\\
\noindent \textbf{Reference for Michigan Magellan Fibre System (M2FS).}

\textbf{Author's response :} \\    
    
\noindent I added the reference for M2FS.\\


\item   Referee's comment : \\
\noindent \textbf{Section 6.2.1}
\noindent \textbf{P66; Figure 6.1}\\
\noindent \textbf{Same comment as Figure 5.1.}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I made the necessary changes in the caption of Figure 6.1 and also added few lines in Section 6.2.1.\\


\item  Referee's comment: \\
\noindent \textbf{Section 6.3}
\noindent \textbf{P67}\\
\noindent \textbf{``For our work, we have taken the J-factors of Tuc-II, Ret-II and UMi from Evans et al., 2016
[12].'' This is repeat of what is already stated in the same section/paragraph.}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I removed this sentence.\\

\item   Referee's comment : \\
\noindent \textbf{P71}\\
\noindent \textbf{Give the reference for T-TEST here.}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I added the reference for T-TEST.\\

\item   Referee's comment : \\
\noindent \textbf{Section 6.4.2}
\noindent \textbf{P73}\\
\noindent \textbf{``Among all sort of above-mentioned background sources,'' to ``Among these'',}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified the sentence.\\

\item   Referee's comment : \\
\noindent \textbf{Section 7.2}
\noindent \textbf{P87: Table 7.1}\\
\noindent \textbf{The table caption should be more explicit mentioning the quantities given in the columns.}

\textbf{Author's response :} \\    
    
\noindent Like the referee’s suggestion, I modified Table 7.1.\\

\end{enumerate}



==> chapters/chapter12__copy_.tex <==
\section{Discussion and Concluding Remarks}

\noindent Finally, we arrive at this chapter to wrap up the thesis. We have performed a detailed study regarding the influence of five component model of elliptical galaxies on Bondi-type spherical or quasi spherical inflow / outflow solutions. Although, we summarized our outcomes at the end of each chapter, we briefly touch up again for the sake of completion. Let us take a quick look back at what has been accomplished so far and what may be possible going forward.

\noindent In our work for Triangulum-II, we have analysed nearly seven years of \texttt{Fermi-LAT} $\gamma$-ray data but could not observe any $\gamma$-ray excess from the location of Tri-II. We then derived the upper limit of $\gamma$-ray flux for two possible scenarios, such as for $\rm{\sigma_{v}= 4.2~km~s^{-1}}$  and $\rm{\sigma_{v} = 3.4~km~s^{-1}}$. For $\rm{\sigma_{v}= 4.2~km~s^{-1}}$, Tri-II constrain the mSUGRA and the MSSM models with low thermal relic densities, whereas the limits constraint the Kaluza-Klein DM in UED and the AMSB models for masses $\lesssim 230$~GeV and $\lesssim 375$~GeV, respectively. Even for $\rm{\sigma_{v} = 3.4~km~s^{-1}}$, Tri-II can constrain the MSSM model with low thermal relic densities and the AMSB model for masses $\lesssim 300$~GeV. Besides, from our work, we found that $\gamma$-ray data from Tri-II can even put stronger limits on the theoretical DM models than UMi. We would also like to point out that our results are entirely based on the standard NFW profile and we do not consider any effects of boost factor related to substructures in Tri-II or the Sommerfeld effect in accord to the annihilation cross-section. Finally, from our work, we can state that with more precise observations of Tri-II, in future we can establish Tri-II as a very strong DM candidate for indirect DM searching.\\

\noindent In case of Tucana-II, we have studied nearly nine years of \textit{Fermi}-LAT data from the location of Tuc-II to investigate the signatures of DM annihilation. We have detected a very faint $\gamma$-ray excess from the location of Tuc-II for both the power-law spectra and the $\gamma$-ray spectrum from DM annihilation. We would also like to report that for $\gamma$-ray spectrum from DM annihilation, we have shown the variation of the TS values for Tuc-II with DM mass. We have also observed that for nine years of \textit{Fermi}-LAT data, TS value of Tuc-II peaks at 
~$m_{DM}\sim$~14 GeV for $100\%$ $b\bar{b}$ annihilation channel, while for $100\%$ $\tau^{+}\tau^{-}$ TS value peaks at $m_{DM}\sim$~4 GeV. In case of our Galactic Center, $m_{DM}$ range between 8 GeV to 15 GeV for $\tau^{+}\tau^{-}$ annihilation channel and the $m_{DM}$ range between 25 GeV to 70 GeV for $b\bar{b}$ annihilation channel play a crucial role to understand the $\gamma$-ray emission possibly arising from DM annihilation \cite{Gordon:2013vta, Hooper:2013rwa, Daylan:2014rsa, Zhou:2014lva, Calore:2014xka}. The mass range for our obtained TS peaks from the analysis for Tuc-II are slightly lower than the mass range required to describe the DM interpretation for Galactic Center. \\

\noindent From our analysis, we have also confirmed that excess from Tuc-II location is increased with increasing the time periods of data and such increase in TS peak value is approximately
proportional to $\sim\sqrt{t}$ \cite{Charles:2016pgz}; here t is the time periods of Fermi-LAT dataset. The most encouraging result of this analysis is  that such successive increase in TS peak values of Tuc-II with larger time periods of the dataset can hint at the existence of any real signal either associated with any astrophysical scenario or resulting from DM annihilation. In the field of indirect DM detection, such hints of $\gamma$-ray emission from Tuc-II may open a new path in DM physics. \\


\noindent When we assume the $\gamma$-ray spectra for DM annihilating to 100$\%$ $\tau^{+}\tau^{-}$ channel, we have obtained a p-value of $\approx$ 0.003 from Tuc-II location corresponding to the background models provided by Fermi-LAT. It can be the result of rare statistical fluctuation in background. The one most tantalizing explanations of such excess are the presence of any surrounding unresolved bright sources. Among different types of unresolved sources, blazars are believed to be the main source of background fluctuation that emits $\gamma$-ray emission just below the threshold limit for Fermi-LAT. We have searched the BZCAT and the CRATES catalog, have found that three nearby radio sources liewithin $1^{\circ}$ ROI of Tuc-II and among all of them, the most nearby source i.e., J225455-592606 lies at just $0.55^{\circ}$ away from the location of Tuc-II. We have also checked the 4FGL catalog of Fermi-LAT (\cite{Fermi-LAT:2019yla}) and have noticed that a source, 4FGL 2247.7-5857 lies 0.66 degree away from Tuc-II location. Hence, it is very unlikely that the emission detected from Tuc-II location would be extremely contaminated by these nearby sources. \\


\noindent We have generated the residual TS maps of Tuc-II for energy $>$ 100 MeV (Figs.~6.4 and 6.5). From these residual TS maps, we have noticed an excess of TS value $\approx$ 6.5 
that is $0.18^{\circ}$ from the location of Tuc-II. We have also shown that whenever we have included Tuc-II to our source model, the excess from that location is greatly reduced. Thus, there is a very high chance that such emission is associated with Tuc-II. We have generated our all residual TS maps for energy $>$ 100 MeV. But the PSF of Fermi-LAT is comparatively large at lower energies, while at higher energies (say for around energy $>$ 500 MeV), the 68$\%$ of the photons would be confined within 1 degree of the location of the source \footnote{\tiny{http://www.slac.stanford.edu/exp/glast/groups/canda/lat{\_}Performance.htm}} Thus, to again check the origin of the excess near Tuc-II location, we have produced a residual TS map for energy $>$ 500 MeV. Interestingly, from this new TS map (Fig 6.11), we could find that after including the Tuc-II to our source model, the nearby excess region has almost disappeared \cite{Bhattacharjee:2018xem}. This signature would probably hint that in Figs.~6.4 and 6.5 after including Tuc-II to source model, the remaining excess emission is associated with weak background modellings. Thus, from our result, we can at best conclude that the nearby excess is associated with Tuc-II location and it might indicate a DM annihilation signal from our Tuc-II \cite{Bhattacharjee:2018xem}.\\


\noindent Several Fermi collaboration papers observe that in a large region of the blank sky, the excess of TS $>$ 8.7 is very common. If we only consider the blazars within $1^{\circ}$ from the location of source, they would roughly account for 10$\%$ of such excesses. The DM subhalos may also be responsible for a $\approx$5$\%$-10$\%$ irreducible background. Therefore, we have re-calibrated our obtained significance and it decreases the TS peak value of Tuc-II from 8.61 to 4.79, i.e., from p value 0.003 to 0.029. At present, with nine years of data, the obtained emission from Tuc-II is much weaker than Fermi-LAT's threshold detection. But from our work, we have also found that the significance of Tuc-II is increased with an increase in time periods of data and from TS map we have also observed a localized excess just beside the Tuc-II. So, in future, with even more time periods of data and with better background modelling, we can expect to explain the origin of the $\gamma$-ray excess from the location of Tuc-II.

\noindent As we have already reported, the excess observed from Tuc-II location is below the detection threshold for Fermi-LAT. Thus we have derived the possible upper-limit of pair-annihilation $<\sigma~v>$ of the DM in Tuc-II as a function of DM mass and five annihilation channels. For our purpose, we have adopted the values J-factor and their uncertainties 
from Evans \textit{et al.}, 2016 \cite{Evans:2016xwx}. \\

\noindent For this, we have analysed the larger periods of compared to other previous works performed on Tuc-II and thus from our analysis, we can expect to provide more stringent limits on the theoretical models. We have observed that for median J-factor value, Tuc-II has imposed a strong constraint on the blue points in both the mSUGRA and the MSSM model, while the 
uncertainty band of Tuc-II have begun to constrain the red points. Because of the large uncertainty band, we may not obtain any impressive limits from Tuc-II in parameter space of ($\sigma v$, $m_{DM}$) but our obtained results stress that with a more detailed understanding of the internal structure, there is a high possibility that in future Tuc-II would provide very strong bounds on theoretically favoured DM models. From results show that for $>$100 GeV DM mass, Tuc-II imposes a stronger bound than the limits obtained from Ret-II. Thus, we can expect if we would have larger periods of dataset and more detailed information of the internal structure,  we should be able to reduce the uncertainty band of Tuc-II to a possible narrow band in parameter space of 
($<\sigma~v>$, $m_{DM}$). Then Tuc-II might be considered as one of the most DM dominated UFDs.


\noindent For this work, we have studied for nearly nine years of LAT data but have not detected any emission from the location of LSB. With DMFit tools, we estimated the $\gamma$-ray and $<\sigma v>$ upper limits for four annihilation states. But because of their low J-factors, individual limits obtained from the LSB galaxies have not put any stringent limits on the DM theoretical models. With the hope of increasing the LAT sensitivity, we have then performed the joined likelihood on the set of four LSB galaxies. As expected, the stacking method has improved the $<\sigma v>$ by the factor of 4 than the individual limits obtained from LSB galaxies. But, the combined $<\sigma v>$ were still around two orders of magnitude weaker than the $<\sigma v>$ limits obtained from refs.~Ackermann et al.\cite{Ackermann:2015zua} and Steigman et al.\cite{Steigman:2012nb}. \\

\noindent The observation data for our chosen LSB galaxies could not particularly favour cored profile over the cuspy profile. The rotational curves for LSBs are in an agreement with the prediction from $\lambda$CDM and some study also indicated that the cuspy profile could also provide a reasonable fit to the DM distribution at the internal core. Thus, motivated by all the 
observation indications, we have modelled the DM distribution of LSB galaxies with the NFW profile. We have also performed a comparative study between NFW, ISO and BURK DM density profiles (check Fig.~7.13) and find that the $<\sigma v>$ limits for each density profiles are overlapping with other. Thus, from our study, we could not favour one profile between all three but for the median value of J-factor, the most stringent limits would come from the NFW profile.\\

\noindent For this study, we have used the multiwavelength approach which is considered as the complementary of the $\gamma$-ray detection method and is very popular in nowadays for the indirect searching of the DM signal. For our analysis, we have preferred to focus on the radio signal and for that purpose, we have followed the code RX-DMFIT. RX-DMFIT is the extension of DMFIt package and is specially designed to investigate the possible radio and X-ray emission from DM annihilation. LSB galaxies have very low nuclear activity and poor star formation rates and that makes them suitable targets for examining the diffuse radio emission most possibly coming from the DM annihilation/decay. We have estimated the multiwavelength SED plots for LSB galaxies and have also checked how the nature of SED varies with varying the parameter sets (check Figs.~7.8 $\&$ 7.9). We have searched for the radio flux limits for all LSB galaxies from  the NVSS sky survey data but only the location of UGC 11707 gives detected flux density values and other thee LSBs only provide the upper limits to the flux density. With the VLA flux density, we have tried to predict the radio $<\sigma v>$ limits in parameter space of ($<\sigma v>$, $m_{DM}$) (check Fig.~7.10). If we consider the 2$\sigma$ uncertainty band associated with the radio limits, we have noticed that the radio limits are overlapping with the limits obtained from stacking analysis for LAT data (check Fig.~7.11) and all three annihilation channels have shown the same nature. Hence, from our analysis, we could, at best, comment that the radio data is competitive with the gamma-ray data. With more detailed observational data and precise analysis, in future, it might be possible for LSB galaxies to impose strong limits on DM models.\\

\noindent We have checked whether with the next generation radio (SKA) and gamma-ray (CTA) telescopes it would be possible to detect any emission from the location of LSB galaxies. We have noticed (check 7.12) that SKA might be able to detect the emission from the location of LSB galaxies and its 1000 hours of observation would have the highest possibility to detect the emission from LSBs. But we would also like mention that in order to claim that SKA would detect the emission from DM annihilation, we first need to perform a simulation study. Besides, the estimated radio emission is also dependent on the various astrophysical scenario. We need to have a well-defined knowledge on the distribution of diffusion zone, magnetic fields, DM density profile, etc.. Hence, from our analysis, we could, at best, hint the possibility of observing the radio signal from LSB galaxies by SKA. We have also found (Fig.~7.14) that for energy ranges between 100 GeV to 1 TeV, it might be possible for CTA to observe the $\gamma$-ray emission with the 50 hours of sensitivity curve. But like SKA, the same conclusion also holds for CTA. A simulation study is needed to examine whether it would be possible for CTA to detect the emission resulting 
from the DM annihilation/decay.\\

\noindent Hence, from our work, we can conclude that the $\gamma$-ray data obtained from the Fermi-LAT could not impose the strong $<\sigma v>$ limits on the WIMP models. We find that the radio signal possibly originated from WIMP annihilation is quite competitive with the $\gamma$-ray emission observed by the Fermi-LAT. Our analysis, at best, indicates that to study $\gamma$-ray and radio signal from the LSB galaxies, SKA and CTA would play a very significant role in 
future. 

\noindent The UFDs, dominated by the DM content, can also possess the moderately large value of the magnetic field and that makes them an ideal target for the indirect detection of DM signals through the multiwavelength approach. In recent times, several literatures have tried to derive the strong limits on annihilation $\langle \sigma v \rangle$ from gamma-ray and radio data \cite{Hoof:2018hyn, DiMauro:2019frs, Fermi-LAT:2016uux, Beck:2019ukt, Regis:2017oet, Regis:2014tga}. For our work, we have considered the newly discovered UFDs detected by the observations performed by Pan-STARRS, DES and some other spectral survey \cite{Bhattacharjee:2020phk}. Using both the gamma-ray (detected by Fermi-LAT) and the radio data (detected by VLA and GMRT), we have searched for the WIMP annihilation signal in 15 UFDs. We have also predicted the possible spectra associated with the radio emission and have checked whether it would be possible for SKA to detect any emission from them \cite{Bhattacharjee:2020phk}.

\noindent With eleven years of Fermi-LAT data, we have not detected any significant emission from the location of UFDs. Thus, we have then derived the upper limits on $\langle\sigma v\rangle$ as a function of DM mass for our chosen DM annihilation channels. We have estimated the limits for 12 UFDs. Because, for Triangulum II, Hydra II and Tucana III, we only have the upper limits on J-factor, so they could not provide any robust limits on the parameter space of ($m_{DM}$, $\langle\sigma v\rangle$) \cite{Bhattacharjee:2020phk}. For gamma-ray data, Holorologium I provided the most stringent constraints but our obtained limits strongly depend on the distribution of DM. Using the NFW profile, we have derived most of the results. Besides, we have also performed a comparative study between NFW, Burkert and ISO profiles. In view of gamma-ray analysis, the Burkert profile imposed the strongest limits on $\langle \sigma v\rangle$, while the ISO imposed the weakest limits \cite{Bhattacharjee:2020phk}. 

\noindent In view of synchrotron emission, we have considered the radio-flux limits observed by GMRT and VLA and have predicted the respective $\langle\sigma v\rangle$ upper limits for $b\bar{b}$, $\tau^+ \tau^-$ and $\mu^+ \mu^-$ final states. We have compared our obtained radio limits with the limits obtained from gamma-ray data and found that the VLA telescope has the potential to impose more stringent limits than Fermi-LAT. 

\noindent We have derived the possible the synchrotron fluxes in UFDs for a wide range of frequencies, i.e., between 10 MHz to 100 GHz and compared these with the sensitivity curves of SKA. We find that for 200 GeV DM mass and $b \bar b$ final state, it might be possible for SKA to detect the radio emission from our considered UFDs, even with its 10 hours of sensitivity curve. For $\tau^+\tau^-$ and $\mu^+ \mu^-$ final states, the emission could be detected with the 100 hours of exposure curve of SKA. On the other side, for comparatively heavy DM masses, (say $\sim$ 2 TeV), the synchrotron spectrum would become harder, and thus a longer observation time would be necessary to detect the radio signal. 

\noindent We also need to remember that the synchrotron fluxes have strong dependences on several astrophysical components, such as magnetic field, diffusion coefficient, distance, etc. But, due to insufficient observation, the values are not very precise. Thus, in order to predict the synchrotron fluxes in UFDs, we must have the most accurate information of the astrophysical parameters, especially the magnetic field and the diffusion coefficient. We have checked how the synchrotron flux in Tucana II varies with $B$, $D_0$ and $\gamma_D$ for DM mass 200 GeV and $b\bar{b}$ annihilation channel. We have noticed that synchrotron emission strongly depends on these. Besides, the emission is also controlled by the choice of DM density distribution in UFDs. We have found that for Tucana II, NFW density profile could produce the maximum amount of radio flux between all three density profiles. Our considered UFDs process a large uncertainties in $r_{1/2}$, $d$ and $\sigma$. The uncertainties in these astrophysical parameters can also affect the synchrotron emission arising from UFDs. We have performed the respective checks and have found that the largest contribution is coming from the uncertainties in $\sigma$. 

\noindent Despite the dependence on these uncertainties, we can safely conclude that a very intriguing aspect of indirect searching for DM signal from UFDs has been discussed in our study. In Fig.~8.13, we have compared the most stringent obtained from the VLA sky-survey with the best limits obtained from the Fermi-LAT data for three final states. From Fig.~8.13, we could notice that for $\mu^+ \mu^-$ and $\tau^+ \tau^-$ final states, VLA imposes the better limits that Fermi-LAT, while for $b\bar{b}$ final state Fermi-LAT provides the stronger limits that VLA \cite{Bhattacharjee:2020phk}.


\noindent In view of indirect DM search, we expect that the next-generation $\gamma$-ray telescope, CTA would play a very crucial role. CTA would have the deepest sensitivity for a very wide range of energies\cite{CTAConsortium:2018tzg} and would be able to investigate the thermal $\langle \sigma v \rangle$ rate from several of DM rich targets. Along with the CTA, in radio sky, SKA is expected to become the most sensitive radio telescopes in the future. Besides, Low-Frequency Array (LOFAR) such as MeerKAT and ASKAP would also be complementary to the CTA and SKA. We can, at best, expect that all of these next-generation telescopes would be able to solve several crucial aspects of dark matter physics.


==> chapters/chapter8.tex <==
\section{Introduction}
\label{sec:intro}
The presence of an abundant non-baryonic dark matter (DM) component in
our universe has not only been established through a variety of
independent observations\cite{Peter:2012rz}, but is also expected to
have played a key role in the evolution of structure at a multitude of
scales\cite{Primack:1997av}.  While a particulate nature of the DM is
called for, such an interpretation necessitates physics beyond the
Standard Model (SM) not only in terms of the identity of the said
particle, but also in terms of the dynamics that determines its relic
density. Several different classes of scenarios have been proposed
with the WIMP (Weakly Interacting Massive Particles) paradigm being
one of the most theoretically appealing ones. This is so because not
only are the parameters (masses and couplings) naturally at the
electroweak scale, but the very interaction that decides the relic
density of the DM particle $\chi$ (largely through processes like
$\chi\chi \to {\cal SS}$, where ${\cal S}$ is a generic SM field)
would also render amenable their detection in terrestrial
experiments \cite{Lisanti:2016jxe,Goodman:Witten,Schumann:2019eaa}.
While much effort has gone into theoretical studies that seek to
reproduce a relic density commensurate with what the cosmological data
suggests, unfortunately no confirmatory signals have been seen in any
laboratory experiments. These include not only dedicated {\em Direct
Search} experiments (based on $\chi {\cal S} \to \chi {\cal
S}$)~\cite{Angle:2008we, Aprile:2016swn,
Aguilar-Arevalo:2016ndq,Amole:2017dex,Cui:2017nnn,Akerib:2017kat,Agnes:2018ves},
but also those at collider facilities (exploiting, typically ${\cal
S}_1{\cal S}_2 \to \chi\chi {\cal S}_3$) , whether it be the
LHC~\cite{Kahlhoefer:2017dnp}, or low-energy facilities such as
Belle~\cite{Borodatchenkova:2005ct, Seong:2018gut,Choudhury:2019sxt}
or Da$\Phi$Ne~\cite{Borodatchenkova:2005ct}. Such non-observation
tends to militate against the requirements for obtaining the correct
relic-density, calling into question the entire paradigm. It should be
realised, though, that event rates in such terrestrial experiments are
governed by many assumptions about the nature of the interaction ({\em
e.g.}, spin-dependence) or the identity of ${\cal S}$ for the dominant
process. For example, if ${\cal S}$ were a third generation fermion,
the signal rates would be quite suppressed, without unduly affecting
cosmological evolution. Similarly, if $\chi$ were very heavy, not only
would production at colliders be suppressed, but the consequent
reduction in its number density (so as to maintain the requisite
energy density) would also suppress the direct detection rates.


This, then brings us to the realm of indirect searches, nominally
carried out through satellite-based and ground-based
experiments~\cite{Buckley:2013bha,Gaskins:2016cha,Fermi-LAT:2016uux,Colafrancesco:2015ola,Acharyya:2020sbj}.
The DM particles in open space can annihilate into a pair of SM
particles and impinge on space-based detectors either directly, or at
the end of a cascade of decays. Free from the aforementioned
suppressions that often plague the other avenues, indirect searches
proffer one of the most promising ways to not only detect the DM, but
also to determine its
properties. Signatures~\cite{Fermi-LAT:2016uux,Ahnen:2016qkx,TheFermi-LAT:2017vmf}
include anomalous photon, positron or antiproton production that could
be observed over and above known astrophysical sources.


In this paper, we concentrate on photon signals, which serve to
provide some of the most robust and stringent constraints on DM
annihilation into a variety of final
states~\cite{Bringmann:2012ez,Cirelli:2015gux}. As can be easily
appreciated, the simplest and most unmistakable signal would be
monochromatic photon emission resulting from either a two body final
state (where the second particle need not be a photon) or from
internal
bremsstrahlung~\cite{Bergstrom:2004cy,Bergstrom:2004nr,Bergstrom:2005ss,
Bringmann:2007nk,Bringmann:2011ye}. Of course, since the DM is electrically
neutral\footnote{While millicharged DM can be accommodated in a
specific class of models, we shall not consider such.},
pair-annihilation into a two-body state with a photon can proceed only
as a loop-level process. A second possibility exists, though, in the
form of, say, $\chi \chi \to e^+ e^-$ with the positron subsequently
annihilating with a low-energy (and astrophysically produced)
electron to lead to a nearly monochromatic photon line. In either
case, the effective cross section is small.


Much larger cross sections are obtained for processes that lead to a
gamma-ray continuum (rather than a line
emission)~\cite{Colafrancesco:2005ji, Colafrancesco:2006he}. These
can, roughly, be divided into two classes, namely
\begin{itemize}
\item {\em prompt emissions} from dark matter annihilations
into any SM pair ${\cal S \bar S}$, with photon(s) being either
radiated off or emanating from the decay of a particle that has arisen
either directly from a primary decay product or as a result
of its hadronization (such as $\pi^0 \to \gamma\gamma$). The photon 
energy could range from $E_{\rm max}\, (M_\chi)$ all the way down.
\item {\em secondary emissions}  from the 
(quasi)stable, charged particles
produced in the primary annihilation event.
Inverse Compton scattering of relativistic particles with the cosmic microwave
background radiation (CMBR) as well as starlight can give photons with energies in the X-ray band, whereas in the presence of astrophysical magnetic fields,
synchrotron radiation (typically in the radio band) result.
\end{itemize}
Various astrophysical systems can be used to look for those
aforementioned signal of DM. For example, the central region of
ordinary Galaxies (like our own Milky Way or M31) are considered
interesting arenas for WIMP searches. Signals from these galactic
central (GC) regions may also be used to understand the well known
{\it cusp/core} issue of the innermost part of the DM distribution
profile. However, photon signals of DM annihilation in the GC region
can be contaminated by galactic diffuse emissions as well as
electromagnetic radiations from various other nearby astrophysical
object such as supernova remnants, pulsars etc.  Owing to such 
unresolved backgrounds, GCs are not ideal for 
effecting precision studies~\cite{Petrovic:2014xra, Gaggero:2017jts, Gaggero:2015nsa,
Cholis:2015dea, Carlson:2015ona}.

N-body simulations indicate the existence of a large number of
DM-dominated sub-halos around typical galaxies~\cite{Kuhlen:2009jv,
Drlica-Wagner:2013bhh}. Some of these sub-halos might be massive
enough to host a dwarf galaxy \cite{Kuhlen:2009jv}, and these appear
as dwarf spheroidal galaxies (dSphs). Constituting the largest
galactic substructures around the Milky Way, these dSphs are expected
harbour the densest DM distributions in the galactic halo, with a
mass-to-light ratio lying in the range (100–1000) $M_{\circ}
/L_{\circ}$, where $M_{\circ}$ and $L_{\circ}$ are the solar mass and
the solar luminosity respectively. Their overwhelming DM content,
minimal Galactic foreground emission, and lack of astrophysical
radiation \cite{Mateo:1998wg, Grcevich:2009gt} render the dSphs
promising targets for the indirect detection of DM.

We consider, here, electromagnetic radiation over a wide range, from gamma down to radio frequencies, emanating from 
dSphs.
Surrounded by large-scale magnetic fields, the sheer size 
thereof confines the $e^\pm $ produced by WIMP annihilation
long enough for these to radiate substantially. Since
the dSphs targeted by the \textit{Fermi} Large Area
Telescope (Fermi-LAT) gamma-ray searches have no 
millisecond pulsars associated with them \cite{Winter:2016wmy},the astrophysical gamma-ray background is essentially negligible. 
%the dSPhs offer natural sites for enhanced rates for the 
%aforementioned annihilations and the subsequent radiations. 
Consequently, the non-observation of such high energy gamma-rays or 
radio-emission 
from nearby dSphs may be used to put strong constraints on the dark
matter annihilation/decay rates.  A decade after the Sloan Digital Sky
Survey (SDSS) revealed a population of ``ultrafaint'' dwarf galaxies
(UFD) in the northern hemisphere (e.g., \cite{Willman:2004kk,
Zucker:2006he, Belokurov:2006ph}), a new generation of sky surveys has
begun charting the southern hemisphere. In
the past few years, nearly two dozen UFDs have been discovered using
data from Pan-STARRS (\cite{Laevens:2015kla, Laevens:2015una}), the
Dark Energy Survey (\cite{Bechtol:2015cbp, kim:2015abc, Kim:2015ila,
Koposov:2015cua}), and other surveys using the Dark Energy Camera at
Cerro Tololo (\cite{Kim:2015xoa, Kim:2016cgf, Kim:2015ghi,
Martin:2015xla}).

Their small halo mass and negligible baryonic
mass render UFDs extremely valuable laboratories
for exploring the nature of dark matter. The southern UFDs provide new
opportunities to address unanswered old questions about the nature and
origin of Galactic substructure, and, in particular, the galactic
luminosity function.  While the latter continues to be revised, its
faint end sets boundary conditions for galaxy formation within a given
cosmological model (\cite{Koposov:2009ru}).

Due to their proximity, high dark-matter content, and the apparent
absence of non-thermal processes, the Milky Way dwarf spheroidal
satellite galaxies are excellent targets for the indirect detection of
dark matter (\cite{Evans:2003sc,Bonnivard:2015xpq}).  To this end, we analyse nearly eleven years of gamma-ray
data collected by the space-based \textit{Fermi} Large Area
Telescope \footnote{http://fermi.gsfc.nasa.gov}. 
In particular,
we consider fourteen recently discovered dwarf spheroidal
galaxies. Amongst them, 13 dSphs are Milky Way satellites and one
(Eridanus II) is from the Local field (LF) (Local Field dwarf
spheroidal galaxies are not bound to Milky Way and M31).

The remaining of the paper is organized as follows: in Section \ref{sec:gamma_flux}, we
describe the different components of the $\gamma$-ray flux and 
the astrophysical $J$-factor for the different dSphs. This is followed, in
Section \ref{sec:DM_profile}, by a discussion
of different possible dark matter profiles, and the consequent $J$-factors.  In
Section \ref{sec:analysis}, we analyze the Fermi-LAT data
for different dwarf spheroidal galaxies to obtain 
upper limits on the annihilation
cross sections for different channels. We also examine
the uncertainty accruing from the determination of
astrophysical parameters and the choice of the dark matter profile.
In Section \ref{sec:synchr}, we focus on the synchrotron radiation from the 
dwarf spheroidal galaxies, especially in the context of the existant 
radio telescopes such as from Giant Metrewave Radio Telescope (GMRT) and Very Large Array (VLA) telescope and the projected sensitivity of the
Square Kilometer Array (SKA). We calculate the upper limits on the DM annihilation cross section using the radio flux upper limits from GMRT and VLA. 
We calculate the synchrotron flux for the dwarf spheroidal galaxies and compare them with the sensitivity curves of SKA.
In Section \ref{sec:synchrotron_uncertainty} we study the
uncertainty in the predicted synchrotron flux because of the
uncertainties in different astrophysical parameters.  We discuss our
conclusions in Section \ref{section:conclusion}.

\section{Source details}\label{section:source_details}

\noindent In Table~\ref{table:astro_fundamental_param_dwarfs}, we have described the properties of the dwarf spheroidal galaxies considered in our study. We have principally chosen all those dwarf galaxies because of their very high mass to light ratio and moderately large velocity dispersion of their member stars. The high mass to light ratio and the large velocity dispersion value generally conform that the UFDs might be very rich in dark matter contents \cite{Baumgardt:2008zt}.  \\

\noindent The properties of our selected dwarf galaxies obtained from their corresponding spectroscopic and the photometric studies are mentioned in Table~\ref{table:astro_fundamental_param_dwarfs}. From this Table~\ref{table:astro_fundamental_param_dwarfs}, $M_{\odot}$ and $L_{\odot}$ represent the mass and the luminosity of the Sun, respectively. The quantities M/L, d, $r_{1/2}$ and $\sigma$ from Table~\ref{table:astro_fundamental_param_dwarfs} denote the mass to light ratio, heliocentric distance, half light radius and velocity dispersion of each UFD galaxies, respectively. The values are obtained from the Ref.~\cite{Pace:2018tin}. \\

\noindent The Aquarius-II was detected on the fringes of the VST ATLAS and the SDSS surveys (\cite{Torrealba:2016svf} ). The Carina-II was discovered in the vicinity of the Large Magellanic Cloud (LMC) in data from the Magellanic Satellites Survey (MagLiteS) (\cite{Torrealba:2018svf}). The discovery of Draco-II was obtained from the search for compact stellar over-densities in the photometric catalog of the Panoramic Survey Telescope and Rapid Response System 1 (Pan-STARRS 1) 3$\pi$ survey (\cite{Laevens:2015kla}). Eridanus-II, Grus-I, Horologium-I, Reticulum-II, aTucana-IInd Tucana-III were first discovered by the Dark Energy Survey (\cite{Koposov:2015cua}). Ref~\cite{Walker:2016mcs} also confirmed that Tucana-II to be a UFD and not a part of any globular cluster. Eridanus II is one of the most distant and least luminous dwarf discovered by the Dark Energy Survey (\cite{Li:2016utv}). For Grus-I, the most significant outlier which is reported by Ref~\cite{Walker:2016mcs}, is to contain four stars (out of seven measured) with [Fe/H] $>$ -1.4. Hydra-II was found serendipitously in DECam data taken for the Survey of the Magellanic Stellar History (\cite{Martin:2015xla}). This satellite is compact and faint, but well within the realm of dwarf galaxies. Leo-V is spectroscopically confirmed ultra-faint dwarf galaxies but it may experience significant tidal stripping as ember stars of Leo-V orbit the Milky Way (\cite{collins:2017}). Pegasus-III was first observed by the archival SDSS data (\cite{Ahn:2013gms, Kim:2015xoa}) and later its stellar overdensity was confirmed  with  deeper  photometry  from the DECam (\cite{Kim:2015xoa}). The kinematic and chemical properties of Pisces-II obtained by Keck/DEIMOS spectroscopy of stars  suggest that Pisces II is dwarf galaxies (\cite{Kirby:2015ija}). Triangulum-II was first detected by the Pan-STARRS Survey (\cite{Laevens:2015una}). In case of Hydra-II, Triangulum-II and Tucana-III, they may be dwarfs but for which either no spectroscopy has been published or the data are inconclusively included.\\

\begin{table}[!h]
\begin{center}
%\label{Tab-3}
\begin{tabular}{||p{2.5cm}|p{2cm}|p{2cm}|p{1.8cm}|p{2.5cm}|p{2.5cm}||}
\hline 
\hline
Galaxy & M/L $(M_{\odot}/L_{\odot})$ & d (Kpc)  & $r_{1/2}~(pc)$ & $\sigma~(km~s^{-1})$ & $\theta_{max}^o$ \\
\hline
Aquarius~II & $1330^{+3242}_{-227}$ & $107.9^{+3.3}_{-3.3}$ & $123^{+22}_{-22}$ & $6.2^{+2.6}_{-1.7}$ & 0.11134 \\
\hline
Carina~II & $369^{+309}_{-161}$ & $37.4^{+0.4}_{-0.4}$ & $76^{+8}_{-8}$ & $3.4^{+1.2}_{-0.8}$ & 0.23\\
\hline
Draco~II & $501^{+1083}_{-421}$ & $20.0^{+3.0}_{-3.0}$ & $12^{+5}_{-5}$ & $3.4^{+2.5}_{-1.9}$ & 0.1\\
\hline
Eridanus~II & $420^{+210}_{-140}$ & $366.0^{+17.0}_{-17.0}$ & $176^{+14}_{-14}$ & $7.1^{+1.2}_{-0.9}$ & 0.062 \\
\hline
Grus~I & $<~2645$ & $120.2^{+11.1}_{-11.0}$ & $52^{+25}_{-25}$ & $4.5^{+5.0}_{-2.8}$ & 0.093\\
\hline
Horologium~I & $570^{+1154}_{-112}$ & $87.0^{+8.0}_{-8.0}$ & $32^{+5}_{-5}$ & $5.9^{+3.3}_{-1.8}$ & 0.0619 \\
\hline
Hydra~II & $<~315$ & $151.0^{+8.0}_{-8.0}$ & $71^{+11}_{-11}$ & $<6.82$ & 0.08509 \\
\hline
Leo~V & $264^{+326}_{-264}$ & $173.0^{+5.0}_{-5.0}$ & $30^{+16}_{-16}$ & $4.9^{+3.0}_{-1.9}$ & 0.077 \\
\hline
Pegasus~III & $1470^{+5660}_{-1240}$ & $215.0^{+12}_{-12}$ & $37^{+14}_{-14}$ & $7.9^{+4.4}_{-3.1}$ & 0.03049\\
\hline
Pisces~II & $370^{+310}_{-240}$ & $183.0^{+15}_{-15}$ & $48^{+10}_{-10}$ & $4.8^{+3.3}_{-2.0}$ & 0.06861\\
\hline
Reticulum~II & $467^{+286}_{-168}$ & $30^{+2}_{-2}$ & $32^{+3}_{-3}$ & $3.4^{+0.7}_{-0.6}$ & 0.24\\
\hline
Tucana~II & $1913^{+2234}_{-950}$ & $57.5^{+5.3}_{-5.3}$ & $115^{+32}_{-32}$ & $7.3^{+2.6}_{-1.7}$ & 0.225\\
\hline
Tucana~III & $<~240$ & $25.0^{+2}_{-2}$ & $43^{+6}_{-6}$ & $<2.18$ & 0.2\\
\hline
Triangulum~II & $<~2510$ & $30^{+2}_{-2}$ & $28^{+8}_{-8}$ & $<6.36$ & 0.15\\
\hline
\hline
\end{tabular}
\end{center}
\caption{Properties of our selected UFD galaxies (\cite{Pace:2018tin})}
\label{table:astro_fundamental_param_dwarfs}
\end{table}

\section{$\gamma$-ray flux from pair-annihilation of WIMPs}
\label{sec:gamma_flux}
A given scenario may include multiple new WIMP candidates (${\cal
W}_i$), of which perhaps only one could constitute the DM. Indirect
detection of the said WIMPs depends on two key processes : $(i)$ the
pair annihilation of the WIMPs through processes such as ${\cal W}_i
{\cal W}_j \to \sum_k {\cal S}_k $, or $(ii)$ the decay\footnote{In
the second case, clearly ${\cal W}_i$ is not protected by a discrete
symmetry. It could have arisen, for example, from the
pair-annihilation of a $Z_2$-odd DM, namely $\chi\chi \to {\cal W}_i
{\cal W}_j$. It should be realised though that a decaying DM is also
admissible as long as the decay is very slow, as, for example, happens
in gravity-mediated decays~\cite{Arun:2017zap}.} of a WIMP into SM
particles, namely ${\cal W}_i \to \sum_k {\cal S}_k $. In each case, a
bunch of energetic standard model particles result in the final state,
either directly from the aforementioned processes or as a result of
the subsequent decay cascades of the ${\cal S}_k$.  However, it
should be noted that neither of the two processes are a must in a given 
particle dark matter scenario.  Furthermore, they bear relevance (apart from
inthe cosmological context) only if they occur at a rate
that can be detected on various experimental facilities based on the
earth or on satellites. This relevance is, of course, determined jointly 
by their rates and
the detectability (in terms of the final particle identities and the
energies they carry), in such facilities, earth-bound or
satellite-based. These, in turn, are
determined by the details of the underlying particle physics model,
both in terms of the spectrum as well the sizes, or even the
existence, of the couplings.  In addition to these, several
astrophysical input parameters also play a major role in the final
observation (both in the annihilation rate as well as in the
propagation of various standard model particles through the
space). Some of these astrophysical parameters, understandably,
contain large uncertainties rendering any conclusive prediction of the
indirect signature of the dark matter very challenging\cite{Conrad:2014nna}.

In this analysis, we focus on the annihilation of Majorana dark matter
in an almost model independent manner, with the simplifying assumption
that the pair-annihilation proceeds into a single channel alone, with
a $100\%$ probability. The consequent individual
sensitivities/constraints can, then, be convoluted, in a relatively
straightforward manner, to that applicable for a given realistic
model.  The DM annihilation rate per unit volume is given by
$\langle \sigma v\rangle \rho^2_{\rm DM}/2 m^2_{\rm DM}$, where
$\rho_{\rm DM}$ is the density, $\sigma$ the cross section and $v$ the
velocity of the second DM particle in the rest frame of the
first\footnote{For a DM annihilation rate of $\langle\sigma
v\rangle \sim 10^{-26}~{\rm cm^3/s}$---one that is consistent with the
correct relic density for $m_{\rm DM} \sim {\cal O}(10^{2-3})\, {\rm
GeV}$---an observable flux of gamma rays is obtained.}.  The thermal
average $\langle\sigma v\rangle$ is estimated using the knowledge of
particle physics and is model-specific.  On the other hand, assuming
that the DM density has a spherical symmetry (a very good
approximation), the radial dependence of $\rho_{\rm DM}$ is modelled
based on astrophysical observations, as we shall discuss later.  For a
specific energy $ E (\equiv E_\gamma)$, the differential $\gamma$-ray
flux $\phi_{\rm{WIMP}} (E, \Delta \Omega)$ (in units of photons
cm$^{-2}$s$^{-1}$GeV$^{-1}$) lying within a solid angle
$\Delta \Omega$ and having arisen from the annihilations of WIMPs of
mass $m_{\rm DM}$, can be expressed~\cite{Abdo:2010ex} as a product of
two terms, one each accounting for the particle-physics and
astrophysics factors, namely
\begin{equation}
\phi_{\rm{WIMP}}(E, \Delta \Omega)~ = ~ \Phi^{pp}(E) \times J(\Delta \Omega) \ .
\label{eqn:dm_flux}
\end{equation}
The particle physics factor can be written as \cite{Abdo:2010ex}:
\begin{equation}
\Phi^{pp}(E)~ = ~\frac{\langle\sigma v\rangle}{8 \pi ~m^{2}_{\rm{DM}}} \sum_{f} 
\frac{dN_{\gamma,f}}{dE}B_{f} \ ,
\label{eqn:dm_pp}
\end{equation}
where $dN_{\gamma, f}/dE$ is the differential photon spectrum (per
annihilation event) for a given final state '$f$', and $B_{f}$ is the
corresponding branching fraction. Several numerical packages like
Pythia \cite{Sjostrand:2007gs}, DarkSUSY (\cite{Gondolo:2004sc}),
DMFit \cite{Jeltema:2008hf} etc. are designed to estimate differential
photons yields from each annihilation channel. While the selection of
standard model final states, through which annihilation would occur
(e.g. $b\bar{b}$, $\tau^{+}\tau^{-}$, $\mu^{+}\mu^{-}$ etc.), is
theoretically motivated, as stated above, we remain agnostic and
consider only a single channel dominance.
Thus, unless otherwise mentioned, in the rest of the analysis, 
only a single final state $(b \bar b, \tau^+\tau^- , 
\mu^+\mu^-)$ will be considered to have been produced ({\em i.e.}, with $100\%$ probability) 
in a DM annihilation process, and consequent limits obtained on the
cross sections.

\subsection{Astrophysical Factor (J)}

Since the total flux is proportional to the factor $J$, it behoves us
to examine it closely. As we are primarily concerned with pair
annihilations, it should depend on $\rho^{2}_{\rm DM}$.  While the
galactic center, where $\rho_{\rm DM}$ is the largest, is associated
with the highest flux, it is also associated with an intense
astrophysical background. In contrast, the dSphs present features that
make them ideal sources. The typical values of the
$J$-factor \cite{Funk:2013gxa} for the GC are $J\approx
10^{22}-10^{23} {\rm GeV}^2 {\rm cm}^{-5} $, while $J\approx
10^{16}-10^{19} {\rm GeV}^2 {\rm cm}^{-5} $ for dSphs and $ J\approx
10^{15}-10^{19} {\rm GeV}^2 {\rm cm}^{-5} $ for galaxy clusters.

While the aforementioned quadratic dependence is indicative, a true
measure of the effective $J$ involves the line-of-sight (l.o.s)
integration of the same, namely~\cite{Abdo:2010ex}
\begin{equation}
J (\Delta \Omega) = \int \int \rho^{2}_{\rm DM} (r(\lambda)) d\lambda ~ d\Omega 
= 2 \pi \int_{\theta_{\rm{min}}}^{\theta_{\rm{max}}} d\theta  \,
     \rm{sin} \theta \int_{\lambda_{\rm{min}}}^{\lambda_{\rm{max}}} d\lambda \; \rho^{2}_{\rm DM} \left(r(\lambda)\right) \ ,
\label{eqn:Jfactor_analytical}
\end{equation}
where $\lambda$ is the l.o.s
distance and $\theta$ is the angle between the l.o.s and the center of
the UFD. The galactocentric distance $r(\lambda)$ is obtained in terms
of the UFD's distance $d$ from the Sun through
\begin{equation}
r(\lambda) = \sqrt{\lambda^{2} + d^{2} - 2~ \lambda ~d~ \rm{cos \theta}} \ .
\label{eqn:r_lambda}
\end{equation}

The DM density profile in dSphs remain a topic of debate.
Two broad classes are popularly used to fit the observational data,
namely those with a cusp-like profile\cite{Navarro:1996gj} or a cored profile\cite{Burkert:1995yz, Salucci:2011ee, Gunn:1972sv} respectively.
While the lack of sufficient kinematical observationals prevents the
selection of a particular profile type, N-body cosmological
simulations, with the most recent results, favors the cuspy
Navarro-Frenk-White (NFW) form~\cite{Navarro:1996gj}, specially for
dSphs and UFD galaxies. This is parametrized as~\cite{Navarro:1996gj}
%%%
\begin{equation}\label{eqn:density_NFW}
\rho_{DM} (r)=\frac{\rho_{s}r_{s}^{3}}{r(r_{s} + r)^{2}} \ ,
\end{equation}
%%%
where $\rho_{s}$ and $r_{s}$ are the characteristic density and scale
radius respectively. These, as well as another one, namely, $r_h$ (that we would
find useful when we discuss synchrotron radiation in Sec.\ref{sec:synchr})
can be obtained using $d$, $\theta_{max}^0$ and $\sigma$. While
the details can be found in ref.\cite{Evans:2016xwx}, we discuss the relations
briefly.

To begin with, consider the mass $M_{1/2}$ contained within the
half-light radius ($r_{1/2}$) of the dSph and approximately
expressed in terms of $r_{1/2}$ and the dSph velocity dispersion $\sigma$ as
\begin{equation}\label{eqn:mhalf}
 M_{1/2} = M(r_{1/2}) \approx \frac{2.5}{G_N} \sigma^2 r_{1/2}.
\end{equation}
where $G_N$ is Newton's constant. The NFW parameter $r_s$ can
be approximated in terms of $r_{1/2}$, {\em
viz.}
\begin{equation}\label{eqn:rs}
 r_s = 5 \, r_{1/2} \ ,
\end{equation}
whereas $\rho_s$ is given by
\begin{equation}\label{eqn:rhos}
 \rho_s = \frac{M_{1/2}}{4\pi r_s^3}
 \left[\log\left(\frac{r_s + r_{1/2}}{r_s}\right)
       -\, \frac{r_{1/2}}{r_s + r_{1/2}}\right]^{-1} \ .
\end{equation}
The distance to the outermost star of the dSph from the center of dSph is,
of course,
\begin{equation}\label{eqn:rmax}
 r_{\rm max} = d\, \, \sin \theta^\circ_{\rm max}.
\end{equation}
And, finally, the diffusion radius ($r_h$) is
defined as twice the distance of the outermost 
star from the center of the dSph, namely
\begin{equation}\label{eqn:rh}
 r_h = 2 \, r_{\rm max} = 2\, d\, \, \sin \theta^\circ_{\rm max}.
\end{equation}

Using eqns.(\ref{eqn:rhos}--\ref{eqn:rh}) with the values of the
parameters $d$, $\sigma$, and $r_{1/2}$ given in
Table~\ref{table:astro_fundamental_param_dwarfs} of the
Appendix, we calculate the parameters $\rho_s$, $r_s$ and $r_h$ and
list them in Table~\ref{table:astro_param_dwarfs}. The parameters in
Table~\ref{table:astro_param_dwarfs} correspond to the central values
of the parameters in Table \ref{table:astro_fundamental_param_dwarfs}
of the appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!ht]
%\input{Sections/tab_astro_param.tex}
\begin{center}
 \begin{tabular}{c c c c c}
  dSphs        & d(Kpc) & $r_h(Kpc)$ & $\rho_s (GeV/cm^3)$ & $r_s (Kpc)$ \\ \hline
  Aquarius II  & 107.9& 0.42  & 2.27035  & 0.615  \\
  Carina II    & 37.4 & 0.3 & 1.78834 & 0.38 \\
  Draco II     & 20 & 0.07 & 71.73  & 0.06 \\
  Eridanus II  & 366 & 0.792 & 1.454 & 0.88 \\ 
  Grus I       & 120.2 & 0.39 & 6.7 & 0.26 \\
  Horologium I & 87 & 0.188 & 30.37 & 0.16 \\
  Hydra II      & 151 & 0.448 & < 8.244 & 0.335 \\
  Leo V        & 173 & 0.465 & 23.83 & 0.15 \\
  Pegasus III  & 215 & 0.228 & 40.73  & 0.185  \\
  Pisces II    & 183 & 0.438 & 8.93 & 0.24 \\
  Reticulum II & 30 & 0.251 & 10.08  & 0.16 \\
  Tucana II    & 57.5 & 0.452 & 3.6  & 0.575 \\
  Tucana III    &  25 & 0.174 & < 2.296 &  0.215 \\  
  Triangulum II & 30 & 0.157 & < 46.1 &  0.14  \\ \hline \hline
  \textbf{Draco}        & 80.0 & 2.5   & 1.4    & 1.0 \\  \hline
 \end{tabular}
\end{center} 
\caption{ The values of the astrophysical parameters for the 14 newly discovered dwarf galaxies \cite{Pace:2018tin}.
The classical dwarf galaxy Draco is also shown for comparison. 
The parameters in this table correspond to the central values of the parameters in Table \ref{table:astro_fundamental_param_dwarfs}.}
\label{table:astro_param_dwarfs}
 \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Given the measurements of $\rho_s$ and $r_s$, it is a straightforward
task to determine $J$. In Table~\ref{table:table-1}, we present this for a
set of dSphs, adopting, in each case, the standard choices of
$\theta_{\rm min} = 0$ and $\theta_{\rm max}= 0.5^\circ$. Also listed,
for comparison, are the corresponding values listed by Pace {\em et
al.}~\cite{Pace:2018tin}, using an empirical scaling relation motivated by
the analytical work of Evans {\em et al.}~\cite{Evans:2016xwx}.  For the
NFW profile, the empirical relation reads
%%
\begin{equation}\label{eqn:jfactor_pace}
\frac{J(0.5^{\circ})}{GeV^{2}cm^{-5}} \approx 10^{17.72} \left(\frac{\sigma_{los}}{5kms^{-1}}\right)^{4} \left(\frac{d}{100kpc}\right)^{-2}\left(\frac{r_{1/2}}{100pc}\right)^{-1} \ ,
\end{equation}
%%
where $\sigma_{\rm l.o.xs}$ and $r_{1/2}$ denote, respectivly, the
velocity dispersion and the half-light radius of the UFD.  It is worth
pointing out the remarkably good agreement between the exact numerical
result and the empirical formula. Indeed, at the level of accuracy of
our results, the two are virtually indistinguishable. It should be
bourne in mind, though, that a different choice of the density profile
would lead to a substantially different value for $J$, a point that we
would return to at a later section. It should also be noticed that, for certain UFDs, only
upper bounds on the $J$-factor exists. This can be traced to the
insufficiency of the kinematic data, which leads to only an upper
bound on the velocity dispersion and, hence, on the $J$-factor \cite{Bhattacharjee:2018xem}.

\begin{table}[!t]
\centering
%\input{Sections/table_1.tex}
\begin{tabular}{|p{2.5cm}|c|c|c|c|}
\hline \hline
Galaxy & \multicolumn{4}{c|}{$\log_{10}(J/{\rm GeV}^2\, {\rm cm}^{-5})$}
\\
\cline{2-5}
& Pace {\em et al}\cite{Pace:2018tin} & \multicolumn{3}{c|}{Direct Integration}\\
\cline{3-5}
& (NFW) & NFW & Burkert & ISO \\
\hline \hline
Aquarius-II & $18.27^{+0.65}_{-0.59}$ & $18.11^{+0.68}_{-0.63}$   & $18.53^{+0.72}_{-0.66}$ & $18.01^{+0.73}_{-0.66}$ \\     
\hline \hline                                                                                                                
Carina-II & $18.24^{+0.53}_{-0.53}$ & $18.16^{+0.55}_{-0.53}$     & $18.45^{+0.60}_{-0.56}$ & $18.05^{+0.58}_{-0.54}$ \\     
\hline \hline                                                                                                                
Draco-II & $18.97^{+1.29}_{-1.69}$ & $19.07^{+1.33}_{-1.69}$      & $19.54^{+1.35}_{-1.70}$ & $18.90^{+1.34}_{-1.70}$ \\     
\hline \hline                                                                                                                
Eridanus-II & $17.29^{+0.35}_{-0.26}$ & $17.14^{+0.35}_{-0.30}$   & $17.68^{+0.35}_{-0.31}$ & $17.06^{+0.35}_{-0.31}$ \\     
\hline \hline                                                                                                                
Grus-I & $16.87^{+1.52}_{-1.68}$ & $16.94^{+1.57}_{-1.74}$        & $17.48^{+1.60}_{-1.75}$ & $16.76^{+1.54}_{-1.67}$ \\     
\hline \hline                                                                                                                
Horologium-I & $19.25^{+0.79}_{-0.70}$ & $19.01^{+0.83}_{-0.73}$  & $19.37^{+0.85}_{-0.75}$ & $18.73^{+0.85}_{-0.75}$ \\     
\hline \hline                                                                                                                
Hydra-II & $<~17.71$ & $<~17.92$                            &  $<~18.46$   &                    $<~17.84$ \\                                                
\hline \hline                                                                                                                
Leo-V & $17.69^{+0.93}_{-0.99}$ & $17.91^{+1.03}_{-1.06}$         & $18.51^{+1.02}_{-1.08}$ & $17.84^{+1.01}_{-1.07}$ \\     
\hline \hline                                                                                                                
Pegasus-III & $18.41^{+0.89}_{-1.07}$ & $18.46^{+0.94}_{-1.05}$   & $19.06^{+1.02}_{-1.07}$ & $18.39^{+1.03}_{-1.05}$ \\     
\hline \hline                                                                                                                
Pisces-II & $17.31^{+0.97}_{-0.107}$ & $17.53^{+1.02}_{-1.09}$    & $18.10^{+1.04}_{-1.09}$ & $17.45^{+1.03}_{-1.09}$ \\     
\hline \hline                                                                                                                
Reticulum-II & $18.95^{+0.57}_{-0.52}$ & $18.76^{+0.53}_{-0.48}$ & $19.21^{+0.53}_{-0.54}$ & $18.66^{+0.53}_{-0.53}$ \\     
\hline \hline                                                                                                                
Triangulum-II & $<~19.72$ & $<~19.74$                      &$<~20.18$ & $<~19.64$ \\                                                
\hline \hline                                                                                                                
Tucana-II & $19.02^{+0.57}_{-0.52}$ & $18.93^{+0.62}_{-0.58}$   & $19.22^{+0.64}_{-0.61}$ & $18.83^{+0.66}_{-0.62}$ \\     
\hline \hline                                                                                                                
Tucana-III & $<~17.68$ & $<~17.87$                        & $<~18.20$   & $<~17.76$ \\                                                
\hline \hline                                                                                                                
Draco & $18.83^{+0.10}_{-0.10}$ & $18.85^{+0.12}_{-0.12}$       & $19.08^{+0.13}_{-0.13}$ & $18.75^{+0.13}_{-0.13}$ \\     
\hline \hline
\end{tabular}
\caption{The $J$-factors for the various UFDs as obtained by directly integrating
Eq.~\ref{eqn:Jfactor_analytical} for three density profiles and for $\theta_{max}=0.5^{\circ}$.
Also shown, for comparison,
are the values obtained by Pace et al~\cite{Pace:2018tin}, for the NFW profile, using 
an approximate scaling relation.} 
\label{table:table-1}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Dependence of $J$ on the density profiles}
\label{sec:DM_profile}

While the NFW is a traditional benchmark choice for the DM profile
motivated by the $N$-body simulations, its cusp-like nature at the
center of the galaxy is quite different from the alternate cored
profiles. While we would use the NFW for most of our numerical
results, it is an imperative to ensure that the cuspy nature does not
lead to extreme answers, To this end, we examine two examples of the
second category, namely the pseudo-isothermal(ISO)~\cite{Gunn:1972sv}
profile and the one originally proposed by
Burkert~\cite{Burkert:1995yz, Salucci:2011ee}. These are given by 
%
\begin{equation}
\rho_{\rm ISO}(r)=\frac{\rho_{c} \, r_c^2}{r^{2}+ r_{c}^{2}}  \ , \qquad
\rho_{\rm BURK}(r)=\frac{\rho_{B}r_{B}^{3}}{(r_{B}+r)(r_{B}^{2} + r^{2})} 
\end{equation}
%
where $r_B$ and $r_{B}$ represent the respective core radii, whereas
$\rho_{c}$ and $\rho_B$ are the corresponding densities at the very
center.  While $ \rho_{\rm BURK}(r) $ resembles an isothermal profile
in the inner regions $(r \ll r_B)$, for large $r$ it falls off much
faster ($r^{-3}$ versus $r^{-2}$).  As in the case for the NFW
profile, the parameters are to be determined from observational data
related to a given galaxy. Based on the study of DM dominated
galaxies, ref.\cite{Boyarsky:2009rb} has approximately related the
parameters for the three profiles, namely $r_s \simeq 6.1 r_c \simeq
1.6 r_B$ and $\rho_s \simeq 0.11 \rho_c \simeq 0.37 \rho_B$.
% \[
% r_s \simeq 6.1 r_c \simeq 1.6 r_B \qquad {\rm and} \qquad
% \rho_s \simeq 0.11 \rho_c \simeq 0.37 \rho_B \ .
% \]

While $N$-body simulations~\cite{Navarro:2008kc, Wagner:2020opz} tend
to favour a cuspy profile (such as the NFW) over the smooth (and
relatively flat at the center) profiles such as the Burkert or the
ISO, insufficient kinematic data (such as those on rotational curves)
prevent us from strongly favoring any one profile. Indeed, some
observations actually favour cored haloes over cuspy ones. Fortunately
for us, the $J$-factor does not have too strong a dependence on the
choice. Indeed, as Table~\ref{table:table-1} demonstrates, the NFW
profile leads to values that are not too far from the average of those
obtained from the three profiles. In other words, the theoretically
favoured choice leads is also a good representative. 

\section{Analysis of $\gamma$-ray fluxes from dwarf spheroidal galaxies}
\label{sec:analysis}

For our study of the high energy gamma-ray signals, originating from
pair annihilations of DM into SM particles within dSphs, we consider the data from the Large Area Telescope (LAT)
onboard the Fermi observatory. 
The Fermi-LAT is a $\gamma$-ray pair conversion space-based
detector that scans the whole sky for every 3 hours from a low-Earth
orbit of 565 km altitude at a 25.6-degree inclination with an
eccentricity $<$0.01. Launched on June 11, 2008, by the Delta
II Heavy launch vehicle from Cape Canaveral, the principal objective
of the Fermi-LAT was to conduct a long term high sensitivity gamma-ray
observations of celestial sources in the energy range from $\approx$
20 MeV to $>$ 500 GeV \cite{Atwood:2009ez}. 
In our study, we have analyzed almost eleven years of sky
survey data (2008-09-01 to 2019-02-04) from the direction of each
UFDs described in section \ref{section:source_details}.
%%%%%
\subsection{The analysis methodology}

Using the latest version of Fermi ScienceTools (v1.2.1) for our
analysis, we process the data with an improved PASS 8 instrument
response function (IRF), in particular the source class IRF,
$\rm{P8R3\_SOURCE\_V2}$. Furthermore, the tool \textit{`gtmktime'}
has been used to extract the ``good time interval'' data from the
whole dataset. Extracting the LAT data within a $15^{\circ}$ radius of
interest (ROI) around each source, we consider only a limited range
for the reconstructed energy $E$, such as $E \approx [0.1, 300]$~GeV, so as
to reduce possible uncertainties at low energies on the one hand and
background contamination at high energies on the other.  To remove the
possible contamination from the earth albedo, we apply a zenith-angle
cut at $90^{\circ}$ as recommended by the Fermi-LAT analysis team.
With the Earth’s limb lying at a zenith angle of $113^{\circ}$, the
application of a zenith cut at $90^{\circ}$ eliminates a large
fraction of the background atmospheric gamma-rays. 

The binned likelihood analysis for the extracted dataset was performed
with the `gtlike' tool \cite{Cash:1979vz, Mattox:1996zz}. To this end,
we first generate a source model file with the inclusion of all the
sources from the 4FGL catalog \cite{Fermi-LAT:2019yla} within a
20$^{\circ}$ ROI from the position of the `source of interest'. Note
that we have extended the spatial coverage up to $20^{\circ}$ ROI to
account for possible overlapping between the point spread functions of
nearby sources. In addition, to
eliminate the possible background effect resulting from galactic and
extragalactic diffuse emission, we have added the Galactic diffuse
model ($\rm{gll\_iem\_v07.fits}$) and the isotropic extragalactic
diffuse model ($\rm{iso\_P8R3\_SOURCE\_V2\_v1.txt}$) to the source
model. The spectral parameters of all the 4FGL sources
\cite{Fermi-LAT:2019yla} within ROI, as well as the normalization
parameters of two diffuse models have been left free in the fitting
procedure. The rest of the background sources within the
$20^{\circ}~\times~20^{\circ}$ ROI have been kept fixed at their
values given in the 4FGL catalog \cite{Fermi-LAT:2019yla}.
Table~\ref{table:fermi_lat_parameters}, lists all the
parameters used at different stages of the analysis of the data.

\begin{table}
\caption{Parameters used in \texttt{Science Tools} for \textit{Fermi}-LAT data analysis}
    %\begin{center}
    \begin{tabular}{||p{6.8 cm}p{6.8 cm}||}
        \hline \hline
        {\bf Parameter for data extraction} &\\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/extract_latdata.html}}} & & &\\
        \hline\hline
        Parameter & Value & &\\
        \hline \hline
        Radius of interest (ROI) &  $15^{\circ}$\\
        TSTART (MET) & 241976960 (2008-09-01 15:49:19.000 UTC)\\
        TSTOP (MET) & 570987500 (2019-02-04 15:38:15.000 UTC)\\
        Energy Range & 100 MeV - 300 GeV\\
        \textit{Fermitools} version & \texttt{1.2.1}\\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/software/}} 
        \hline \hline
        $~~~~~~~~~~~~~~~~~~~$\texttt{gtselect} for event selection &\\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/help/gtselect.txt}\label{gtselect}}
        \hline \hline
        Event class & Source type (128)\\ 
        Event type & Front+Back (3) \\ %\footref{datacut} 
        Maximum zenith angle cut & $90^{\circ}$\\ %\footref{datacut} 
        \hline \hline
        $~~~~~~~~~~~~~~~~~~~$\texttt{gtmktime} for time selection & \\%\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/help/gtmktime.txt}} 
        \hline \hline
        Filter applied & $\textit{(DATA\_QUAL>0)\&\&(LAT\_CONFIG==1)}$ \\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/data_preparation.html}\label{data_preparation}}$ 
        ROI-based zenith angle cut & No & &\\ %\footref{data_preparation}  
        \hline \hline
        $~~~~~~~~~~~~~~~~~~~$\texttt{gtltcube} for livetime cube &\\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/help/gtltcube.txt}} 
        \hline \hline
        Maximum zenith angle cut ($z_{cut}$) & $90^{\circ}$ \\%\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/documentation/Cicerone/Cicerone_Likelihood/Exposure.html}}$ 
        Step size in $cos(\theta)$ & 0.025\\
        Pixel size (degrees) & 1\\
        \hline \hline
        $~~~~~~~~~~~~~~~~$\texttt{gtbin} for 3-D counts map &\\
        \hline \hline
        Size of the X $\&$ Y axis (pixels) & 140\\
        Image scale (degrees/pixel) & 0.1\\
        Coordinate system & Celestial (CEL)\\
        Projection method & AIT\\
        Number of logarithmically uniform energy bins & 24\\ 
        \hline \hline
        $~~~~~~~~~~~~~~~~~~~$\texttt{gtexpcube2} for exposure map & \\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/help/gtexpcube2.txt}} & & &\\
        \hline \hline
        Instrument Response Function (IRF) & $\rm{P8R3\_SOURCE\_V2}$ \\%\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/documentation/Pass8_usage.html}\label{pass8}}$ 
        Size of the X $\&$ Y axis (pixels) & 400\\
        Image scale (degrees/pixel) & 0.1\\
        Coordinate system & Celestial (CEL)\\
        Projection method & AIT\\
        Number of logarithmically uniform energy bins & 24\\ 
        \hline \hline
        $~~~~~~~~~~~~~~~~~~~$diffuse models and Source model XML file &\\%\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/user/make4FGLxml.py}} & & &\\
        \hline \hline
        Galactic diffuse emission model & $\rm{gll\_iem\_v07.fits}$\\ %\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/access/lat/BackgroundModels.html}\label{background}}$ 
        Extragalactic isotropic diffuse emission model & $\rm{iso\_P8R3\_SOURCE\_V2\_v1.txt}$\\%\footref{background}$ & &\\
        Source catalog & 4FGL & & \\
        Extra radius of interest &  $5^{\circ}$\\
        Spectral model &  DMFit Function\cite{Jeltema:2008hf} \\%\footnote{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/scitools/source_models.html}} & &\\
        \hline \hline
                
    \end{tabular}
    %\end{center}
        \label{table:fermi_lat_parameters}
\end{table} 


To search for the $\gamma$-ray emission coincident with our targets, we
have first modelled our sources with a power-law spectral model ($dN/dE \propto E^{-\Gamma}$) with spectral index $\Gamma$ = 2 \cite{Bhattacharjee:2018xem}. As a statistical discriminator, we use the ratio of the maximum likelihoods
for two hypotheses, namely, $TS = -2\ln\Big(L_{\rm {(max, 0)}}/L_{\rm
  {(max, 1)}}\Big)$, where $L_{\rm {(max, 1)}}$ and $L_{\rm {(max,
    0)}}$ respectivelty denote the maximum likelihood in the presence
of a signal and the null hypothesis. As no gamma-ray signal was observed from the direction of any of the UFDs, we then derive 95$\%$ confidence level (CL) upper limits (UL) on the gamma-ray flux from the region of these objects. To estimate the flux upper limits in 95$\%$ C.L., we use the Bayesian approach (\cite{Helene:1990yi}), as this is more sensitive~\cite{Rolke:2004mj, Barbieri:1982eh} than the profile
likelihood method for low statistics. The approach developed in Ref. \cite{Helene:1990yi} is already implemented in the pyLikelihood module of \texttt{ScienceTools}.


\subsection{Possible DM annihilation Constraint with eleven years of Fermi-LAT data}\label{section:gamaray_sigmav_constraint}

\begin{figure}[h]
  \centering
  %\vskip  -1in
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/flux_bb.pdf}
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/flux_tt.pdf} \\
  \vskip -1in
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/flux_mm.pdf}
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/legend.pdf}
  \vskip -0.5in
  \caption{$95\%$ C.L. upper limits on the $\gamma$-ray fluxes
  (from DM pair-annihilations in UFDs) as a function of
  $\rm{m_{DM}}$. In deriving these, the indicated channel is assumed
  to be an exclusive one.  The curves for Triangulum-II, Hydra-II and
  Tucana-III denote their maximum possible upper
  limits.}  \label{figure:fermi_flux}
\end{figure}


\begin{figure}[h]
  \centering
  %\vskip  -0.5in
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/sigma_bb_scaled.pdf}
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/sigma_tt_scaled.pdf} \\
  \vskip -1.0in
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/sigma_mm_scaled.pdf}
  \includegraphics[width=0.49\textwidth,height=0.44\textwidth]{figures/legend.pdf}
  \vskip -0.6in
  \label{fig:cross_legends}
 \caption{95\% C.L. upper limit on the thermally
 averaged WIMP pair-annihilation $\langle \sigma v \rangle$ as derived
 from the upper limits on the gamma-ray fluxes from individual UFDs.
 In each case, the annihilation channel is assumed to be
 exclusive.
  The curves for Triangulum-II, Hydra-II and Tucana-III, denote their maximum possible upper limits.}
   \label{figure:fermi_cross}
\end{figure}

The aforesaid upper limits on the gamma-ray fluxes from DM
annihilation can be translated to constraints in the two dimensional
plane of the WIMP mass and the thermally averaged pair-annihilation
cross section $\langle \sigma v\rangle$.  This exercise, though,
depends on the final states resulting from the annihilation processes
and, hence, on the details of the model. However, as indicated
at the outset, we adopt an agnostic standpoint and consider three
{\em exclusive} channels, namely $b \bar b$, $\tau^+\tau^-$ and $\mu^+\mu^-$. 

For estimating the flux upper limits in 95$\%$ C.L. and limits to the
$\langle \sigma v \rangle $ of WIMP pair-annihilation, we have fitted the
$\gamma$-ray spectrum arising from the DM-dominated dSphs with an
MC-simulated DM self-annihilation spectrum, DMFitFunction
\cite{{Jeltema:2008hf}}. The DMFit package is based on the particular set
of MC simulations of hadronization and/or decay of the annihilation
products as used by the DarkSUSY \cite{Gondolo:2004sc} team. 

The functional form of DMFitFunction
(modified form of Eq.~\ref{eqn:dm_flux}) can be written as

\begin{equation}\label{eqn:dm_spectrum}
\frac{dN}{dE} (E,\Delta \Omega) = \langle \sigma v \rangle ~ J(\Delta \Omega) (B~F(M_{DM},C_{0}) + (1 - B~F(M_{DM},C_{1}))
\end{equation}

From Eq. \ref{eqn:dm_spectrum},
B, $C_{0}$ and $C_{1}$ define the branching ratio, 
primary decay channel and secondary decay channel,
respectively. The DMFitFunction is implemented in Fermi
\texttt{ScienceTools} as a DMFit package
\cite{Jeltema:2008hf} and the values of F($M_{DM}$,C) are provided by
the Fermi-LAT team. For J-factor, we have taken the values from Pace et al,
2019 (\cite{Pace:2018tin}) (See Table~\ref{table:table-1})

In Fig.~\ref{figure:fermi_flux}, we have shown the variation
of flux upper limits in $95\%$ C.L. of all UFDs with $m_{DM}$ for
$b\bar{b}$, $\tau^{+}\tau^{-}$ and $\mu^{+} \mu^{-}$ annihilation
channels. For all possible annihilation channels, with increasing mass, the spectrum
from WIMP annihilation always shifts to higher energies
\cite{Serpico:2009vz} and so, we can expect that the variation of flux
upper limits would be comparatively less for high $m_{DM}$. From
\ref{figure:fermi_flux}, we can also check the same.

In Fig.~\ref{figure:fermi_cross}, we have displayed the $95\%$
C.L. upper limit of the thermally averaged WIMP pair-annihilation
$\langle \sigma v \rangle $ of UFDs, as a function of the $m_{DM}$ for each of the
annihilation channels mentioned above. 


\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/horologium_cross_comparison.pdf}
 \caption{Variation of $\langle \sigma v\rangle$ upper limits of Horologium-I with $m_{DM}$ for three annihilation final states.}
 \label{fig:horo_cross}
\end{figure}

In Fig.~\ref{figure:fermi_flux} and
Fig.~\ref{figure:fermi_cross}, we have also compared our obtained
upper limits with Draco which is considered as one of the best
candidates for indirect DM detection. Here we would like to
mention that among all our selected dwarf galaxies, Horologium-I
provides the strongest limit (Fig.~\ref{figure:fermi_cross}) for all
three annihilation final states and from our study, we can observe the
limits obtained from Horologium-I can even provide more stringent
limits on the theoretical WIMP models than Draco.

But we should also keep in mind that, due to insufficient kinematics
data, newly discovered Horologium-I might come with large
uncertainties in J-factor and so, we could not firmly state that
Horologium-I is the better candidate than Draco. But, from this
signature, we can expect that in future Horologium-I can come as a
very rich DM dominated galaxy. In subsection~\ref{section:uncertainties_horo_tuc}, we have studied
the uncertainty band in Horologium-I and Tucana-II.

From Fig.~\ref{figure:fermi_flux} and Fig.~\ref{figure:fermi_cross}, the flux upper limits and corresponding $\langle \sigma v \rangle $
limits of Triangulum-II, Hydra-II and Tucana-III can only produce the maximum possible upper limits. 
If we check the Table~\ref{table:table-1}, we can observe that at present 
we can only estimate the upper limits of J-factor for these three UFDs. So, from Triangulum-II, Hydra-II and Tucana-III, 
we can only obtain the limiting values for $\gamma$-ray flux upper limits and $\langle \sigma v \rangle $.

We have taken the Horologium-I from Fig.~\ref{figure:fermi_cross} and in Fig.~\ref{fig:horo_cross}, 
we have displayed the variation of $\langle \sigma v \rangle$ of Horologium-I for three annihilation channels. 
From Fig.~\ref{fig:horo_cross}, we can observe that for $\gamma-ray$ observation $100\%$ $b\bar{b}$ channel provide the more stringent limits than other two final states in the plane of ($\langle \sigma v \rangle, m_{DM}$). All our selected UFDs have showed the same signature like 
Horologium-I for each annihilation channels. Thus, in Fig.~\ref{fig:horo_cross}, we have only
shown the results for Horologium-I.


Next, we check how does the upper limits to the
thermally averaged pair-annihilation $\langle \sigma v \rangle $ can change with
changing the DM density profiles. In section~\ref{sec:DM_profile}, we have already
derived the J-factor for NFW, BURK and ISO profiles. Now, using
Eq.~\ref{eqn:dm_spectrum} and J-factor values from
Table~\ref{table:table-1}, we have also compared the upper
limits to the thermally averaged pair-annihilation $\langle \sigma v \rangle $ of
Horologium-I=I for three density profiles and for this purpose we have
considered the $\rm{100\%~b\overline{b}}$ annihilation channel. From
Fig.~\ref{figure:profile_comparison}, we can observe that all three
density profiles have provided nearly the same order of $\langle \sigma v \rangle $
upper limits. But among them, the BURK density profile can impose the
most stringent $\langle \sigma v \rangle $ upper limit on the theoretical models
whereas ISO profile would produce comparatively weaker limits in the
plane of ($\langle \sigma v \rangle, m_{DM}$) than two other density profiles.

\begin{figure}[h!]
\centering
 \includegraphics[width=0.5\textwidth,clip,angle=0]{figures/density_profile_comparison_horo.pdf}
\caption{Comparison between the $\langle \sigma v \rangle $ upper limits for three density profiles for $100\%$ $b\overline{b}$ final state.}
  \label{figure:profile_comparison}
 \end{figure}


Here we would like to point out that except for Tucana-II, most of our targets have not shown any faint emission from their location (i.e. TS $\preceq$ 5). Thus, here we have only reported the result for Tucana-II. In Table~\ref{table:ts_values}, we have listed the TS peak value of UFDs for $b\bar{b}$ and $\tau^{+}\tau^{-}$ annihilation channels. In our recent publication (ref.~\cite{Bhattacharjee:2018xem}), we have
reported the intriguing hint of faint $\gamma$-ray emission from the
location of Tucana-II. In that paper (\cite{Bhattacharjee:2018xem}),
we have also shown that the TS peak of Tuc-II is increased with the
larger dataset and the same nature is followed by both the $b\bar{b}$
and $\tau^{+}\tau^{-}$ annihilation channels. 

\begin{table}
	\begin{center}
 	\begin{tabular}{|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
 	\hline \hline
  UFDs & $TS_{peak}$ for $b\bar{b}$ & $TS_{peak}$ for $\tau^{+}\tau^{-}$ \\ 
  \hline \hline
  Aquarius II  & 2.88 & 2.94 \\
  Carina II    & 1.24 & 1.81 \\
  Draco II     & 1.37 & 1.88 \\
  Eridanus II  & 0.81 & 1.23 \\ 
  Grus I       & 1.59 & 1.65 \\
  Horologium I & 4.21 & 4.71 \\
  Hydra II     & 2.21 & 2.31 \\
  Leo V        & 0.88 & 0.92 \\
  Pegasus III  & 1.91 & 2.13 \\
  Pisces II    & 1.22 & 1.96\\
  Reticulum II & 4.85 & 4.95 \\
  Tucana II    & 11.87 & 12.47 \\
  Tucana III    &  4.36 & 4.53 \\  
  Triangulum II & 1.19 & 1.25 \\ 
  \hline \hline
  \end{tabular}
\end{center} 
  \caption{TS peak value for two annihilation final states}
  \label{table:ts_values}
  \end{table}

In our present work, we have analyzed nearly eleven years of Fermi-LAT
data and in ref.~\cite{Bhattacharjee:2018xem} we analyzed nearly nine
years of data. So, we can expect that the TS value for Tucana-II would
again increase with eleven years of data. In
Fig.~\ref{figure:ts_tucana}, we have obtained our expected
result. Even though the observed significance with eleven years of
Fermi-LAT data is faint (i.e. TS~$<$~25) to claim anything
strongly. The most encouraging part of this result is that the TS peak
of Tuc-II is continuously increasing with time and in the future, this
could lead us to a detection of a real signal either from any
astrophysical connection or from WIMP annihilation. \\

\begin{figure}[h!]
\begin{center}
 {\includegraphics[width=0.5\textwidth,clip,angle=0]{figures/ts_compare.pdf}}
\caption{The observed TS peak of the excess $\gamma$-ray 
emission from the direction of Tuc-II for four different time intervals of
Fermi-LAT data, whereas, the red and blue markers denote the TS peak for 
$100\%$ $b\bar{b}$ and $100\%$ $\tau^{+}\tau^{-}$ annihilation channels, 
respectively.}
\label{figure:ts_tucana}
\end{center}
\end{figure}



%\subsection{A faint $\gamma$-ray emission from Tucana-II location}

\subsection{Comparison between our obtained result from the Fermi-LAT analysis with the estimated limits provided by Planck}

In the early epoch of the universe, the WIMP annihilation could 
pump in electromagnetically interacting particles into the cosmic bath with
a wide-ranging observable effects. The injection of such charged 
particles could significantly increase the residual ionization fraction which 
in turn modify the last scattering surface as well the observed 
CMB anisotropy\cite{Gruzinov:1998un, Lewis:1999bs}. The WMAP \cite{Bennett_2013}  and most recent the Planck satellite experiments \cite{Aghanim:2018eyx} are 
highly sensitive to capture any such modifications in the CMB. 
Thus, the Planck satellite experiment placed a very 
strong and model-independent limits on aforementioned energy-injections by
the annihilating WIMPs~\cite{Aghanim:2018eyx}. 
This limit on the energy-injections has been 
further translated into the WIMP annihilation cross-section. 
To compare this limit with that of obtained from the Fermi-LAT collaboration,
we choose Horologium-I as our target dSphs and in  
Fig.~\ref{figure:planck_comparison} we display the comparison. From
Fig.~\ref{figure:planck_comparison}, we observe that for the limit 
obtained by the Fermi-LAT Collaboration on the WIMP annihilation 
cross-section for the exclusive $b{\bar b}$ channel 
is better limit than the Planck limits for ${\rm M_{\rm DM}} \sim 10 $ GeV to
10 TeV. On the other hand in the case of exclusive 
$\mu^{+}\mu^{-}$ annihilation channel the Planck Collaboration 
provides the stringent limit comparted to that of give by the 
Fermi-LAT Collaboration. For the $\tau^{+}\tau^{-}$ annihilation
channel, the Fermi-LAT imposes stringent limits 
in the mass range $\lesssim 400$~GeV, while Planck is
likely to impose the most stringent limits on $\langle \sigma v \rangle $ 
in the mass range $\gtrsim 400$~GeV.

\begin{figure}[h!]
\begin{center}
 {\includegraphics[width=.5\linewidth]{figures/comparison_between_fermi_and_planck.pdf}}
\caption{Comparison between the limits obtained for Horologium-I from Fermi-LAT with the limits provided by Planck. }
\label{figure:planck_comparison}
\end{center}
\end{figure}


\subsection{Uncertainty band in Horologium-I and Tucana-II}\label{section:uncertainties_horo_tuc}

The $\gamma$-ray analysis is one of the most popular ways to examine
the indirect detection of DM signature. But the large
uncertainty in J-factors can be a matter of concern. Focusing on the
uncertainty in J-factor is important because the large uncertainty in
J-factor can dominantly weaken the DM particle constraints
(i.e. limits on the cross section).  \\

So, in this section, we have tried to show the variation of 95$\%$
C.L. upper limit of the WIMP pair-annihilation $\langle \sigma v \rangle $ with
increasing $m_{DM}$ for J-factor with its uncertainties. For this
purpose, we have chosen Horologium-I and Tucana-II and have only shown
the variation for $b\bar{b}$ annihilation channel. We have considered
Horologium-I because out of all UFDs it has provided the most
stringent limits. In the case of Tucana-II, we have obtained a faint
emission from the source location \cite{Bhattacharjee:2018xem}, so we
would like to check the variation for Tucana-II. The median J-factor
and its uncertainties are taken from Pace at al, 2019
(\cite{Pace:2018tin}). \\

In Fig.~\ref{figure:crossuncertainty} we have shown the 95$\%$ C.L. upper
limit of the WIMP annihilation $\langle \sigma v \rangle $ for Horologium-I and
Tucana-II. From Fig.~\ref{figure:crossuncertainty} the dashed lines
correspond to the uncertainty in J-factors of each UFDs, while the
solid line depicts the median value of J-factor and the regions
between two dashed lines represent the uncertainty in the DM
density profiles of UFDs.

From Fig.~\ref{figure:crossuncertainty}, it is evident that for Tucana-II
and Horologium-I imposes a large uncertainty band. In the case of
UFDs, very few numbers of stars have been detected so far which is the
main obstacle in understanding the DM distribution in
UFDs. The large uncertainties in J-factor come from insufficient
kinematics data. With the more precise observation of the internal
structure, in the future, we can expect to reduce such uncertainty
band to a possible single upper limit curve of $\langle \sigma v \rangle $ and that
might improve the constraint limit on beyond Standard Model. 

  \begin{figure}[h!]
  \centering
 \includegraphics[width=.45\linewidth]{figures/horologium_uncertainty.pdf}
  \includegraphics[width=.45\linewidth]{figures/tucana_uncertainty.pdf}
  \caption{Variations of 95$\%$ C.L. upper limit of the WIMP pair-annihilation $\langle \sigma v \rangle $ with increasing $m_{DM}$ for $b\bar{b}$ annihilation final states of (a) Horologium-I and (b) Tucana-II. The dashed lines represent the uncertainty in the DM density profiles of UFDs and the solid line denotes the upper limit of $\langle \sigma v \rangle $ in 95$\%$ C.L. corresponds to median J-factor. The colors and the line-styles of different curves are indicated in the diagram}
  \label{figure:crossuncertainty}
 \end{figure}

\section{Synchrotron radiation from dwarf spheroidal galaxies}
\label{sec:synchr}
A charged particle propagating through the interstellar medium would
lose energy owing to a variety of electromagnetic processes such as
inverse Compton radiation, synchrotron radiation, Coulomb losses and
bremsstrahlung. While this applies to any charged particle, the
radiation would be substantial only if the particle is sufficiently
long-lived, or in other words if it is one of $e^\pm$ or $p, \bar
p$. The contributions from the last two are much smaller, both on
account of their larger masses as well as the small probability for a
quark (from the hard process) fragmenting into a $p, \bar p$. Given this,
we develop the subsequent arguments for $e^\pm$ alone. The other
species can be treated analogously.

A complete treatment of the DM-initiated synchrotron radiation must
consider the diffusion and aforementioned energy loss contributions
from the secondary particles. The formalism,
developed
in refs.\cite{Colafrancesco:2005ji, Colafrancesco:2006he, McDaniel:2017ppt},
can
be summarised by the transport equation for $n_e(r,E)$, the number density
of $e^\pm$ of a given energy
$E$ at the position $\mathbf{r}$ with respect to the center of the
dSph), {\em viz.},
\begin{align}\label{eqn:diffusion}
\frac{\partial}{\partial t} \frac{dn_e(r,E)}{dE}
= \nabla . \Big( D(E,\mathbf{r}) \nabla \frac{dn_e(r,E)}{dE}\Big)
     + \frac{\partial}{\partial E} \Big( b(E,\mathbf{r}) \frac{dn_e(r,E)}{dE}\Big)
     + Q_e (E,\mathbf{r}).
\end{align}
Here, $ D(E,\mathbf{r})$ is the space-dependent diffusion coefficient,
$b(E,\mathbf{r})$ encapsulates the energy loss term and the source
term $Q_e$ is given by
\begin{align}
 Q_e (E,\mathbf{r}) = \frac{\rho^2_\chi(\mathbf{r}) \langle \sigma v\rangle}{2 m_\chi^2}    \frac{dN_{e}}{dE},
\end{align}
where $N_e$ is the number of $e^{\pm}$ produced with a given energy $E$
per DM annihilation.

The energy loss term receives several independent contributions
(from the processes listed earlier) and is given by \cite{Colafrancesco:2005ji,McDaniel:2017ppt}

\begin{align}
b(E)  = & b_{IC}(E) + b_{Syn}(E) + b_{Coul}(E) + b_{brem}(E) \nonumber \\ 
      = & b_{IC}^0 E^2 + b_{syn}^0 B^2 E^2  \nonumber \\ 
        & + b_{Coul}^0 n ( 1 + log(\gamma /n)/75) + b_{brem}^0 n (log(\gamma / 
n) + 0.36).
\end{align}

where the dependence on $\mathbf{r}$ has been suppressed.
Here, $B$ is the magnetic field in $\mu G$, whereas $n$ is the number
density of thermal electrons in cm$^{-3}$ and $\gamma = E/m_e$
is the time-dilation factor. 
The various energy loss 
parameters $b^0_{\rm IC}, b^0_{\rm syn}, b^0_{\rm Coul} $ and $b^0_{\rm brem}$
have values $ 0.25,0.0254,6.13$ and $1.51 $ respectively in the units
of $ 10^{-16}$ GeV s$^{-1}$ \cite{Colafrancesco:2005ji}. 
In the absence of detailed knowledge of the structure of the dSph,
the diffusion coefficient $D(E, \mathbf{r})$ may be
assumed to be independent of position. Comparisons of simulations with
data suggest that 
the consequent loss of accuracy is not too severe and that
the form 
\begin{equation}\label{eqn:diffusion_coefficient}
 D(E) = D_{0} \left(\frac{E}{1 \GeV}\right)^{\gamma_{D}}
\end{equation}
may be used.


Assuming spherical symmetry, a uniform magneric field and a uniform
number density of thermal electrons, the stationary state solution of
the diffusion equation is given by
\begin{align}\label{eqn:solutionndifusion}
  \frac{dn_e}{dE}(r,E) = \frac{1}{b(E)} \int_{E}^{M_\chi} dE^\prime \,
            G\Big(r, v(E)-v(E^\prime)\Big) Q_e(E^\prime,r),
\end{align}
where the  Greens function is given by 
\begin{equation}
 G(r, \Delta v)  = \frac{1}{\sqrt{4\pi \Delta v}} \sum_{k=-\infty}^{\infty} (-1)^k 
                     \int_{0}^{r_h} dr^\prime \frac{r^\prime}{r_k}
                     \left(\frac{\rho_\chi(r^\prime)}{\rho_\chi(r)}\right)^2 
                  \left[ \exp\left(-\frac{(r^\prime -r_k)^2}{4 \Delta v}\right)
                     - \exp\left(-\frac{(r^\prime + r_k)^2}{4 \Delta v}\right)
                     \right],
\end{equation}

Here $r_h$ defines the diffusion zone of the dSph, namely the
radius at which the free escape boundary condition $dn_e(r_h,E)/dE =
0$ may be imposed.  Typically, $r_h$ is approximately twice the radius
of the last stellar component of the galaxy ({\em i.e.}, twice the
distance of the outermost star from center).

The synchrotron power spectrum or the total power radiated per unit
frequency at $\nu$ by an electron of energy $E$ present
in a magnetic field $B$, {\em viz.}, $P_{\rm synch}(\nu,E,B)$ is defined as: 
\begin{equation}
 P_{\rm synch}(\nu, E, B) = \pi \sqrt{3} r_0 m_e c \nu_0 \, \int_0^\pi \, d\theta \, \sin^2\theta \, F\big(\frac{x}{\sin\theta }\big),
\end{equation}
where $\theta$ is the pitch angle, $r_0 = e^2/(m_e c^2)$ is the
classical electron radius and $\nu_0 = eB/(2\pi m_e c)$ is the
non-relativistic gyro-frequency. While
\begin{equation}
 F(y) = y \,  \int_y^\infty d\zeta \, K_{5/3}(\zeta) \simeq 1.25 \, y^{1/3}\,
      e^{-y} \, (648 + y^2)^{1/12} \ ,
\end{equation}
the quantity $x$ is given by
\begin{equation}
 x = \frac{2 \, \nu\, m_e^2 \, (1+z)}{3 \, \nu_0\, E^2} 
\end{equation}
with $z$ being the redshift of the source. For the dSphs under consideration,
$z \approx 0 $. 

We can, now, estimate the total energy radiated or the local
emissivity (i.e. the amount of energy radiated at a given
$\mathbf{r}$, per unit volume per unit time) at a given frequency
$\nu$ in the form of synchrotron radiation in terms of $P_{\rm synch}$
and $dn_e/dE$ {\em viz.},
\begin{equation}\label{eqn:emissivity}
j_{\rm synch}(\nu, r)
 = \int_{m_e}^{M_{\chi}} dE \left(\frac{dn_{e^+}}{dE}
 + \frac{dn_{e^-}}{dE}\right) P_{\rm synch}(\nu,E,B) = 
 2 \int_{m_e}^{M_{\chi}} dE \, \frac{dn_{e^-}}{dE}\,
 P_{\rm synch}(\nu,E,B) \ .
\end{equation}
The integrated synchrotron flux density spectrum is, now, given by 
 \begin{equation}\label{eqn:syn_flux}
S_{\rm synch}(\nu) = \frac{1}{4\pi d^2}\int d^3 r \, \,  j_{\rm synch}(\nu,r),  
 \end{equation}
where $d$ is the distance to the dSph and
the integration is over the whole diffusion volume.


\subsection{Synchrotron radiation from the newly discovered dwarf spheroidal galaxies}
As we have seen above, unlike in the case for the
gamma-rays,
the synchrotron flux is not related to the $J$-factor, especially on
account of the dependence on the diffusion and energy loss processes.
Consequently, apart from the particle physics details and the
astrophysical parameters already discussed, the synchrotron flux also
depends on the magnetic field $B$ inside the dSph as well as
the diffusion coefficient parametrized by $D_0$.


Observations indicate that the magnetic field of dSphs are of the
order of 1 $\mu$G
\cite{Colafrancesco:2006he,McDaniel:2017ppt, Spekkens:2013ik}.
Although dSphs in the outer region of the Milky Way's magnetic
field can have magnetic field larger than 1 $\mu$G,
\cite{McDaniel:2017ppt,Natarajan:2015hma}, for our calculations
we assume a uniform profile of strength
$B=1 \, \mu$G~ \cite{Colafrancesco:2006he, Jeltema:2008hf}.

The diffusion coefficient, for which we assume the simplified form of
eqn.\ref{eqn:diffusion_coefficient}, has larger uncertainties. For
galaxy clusters, a value for the coefficient $D_0$ as large as
$10^{28}$--$10^{30}\, {\rm cm}^2/{\rm s}$ have been argued
for~\cite{Natarajan:2015hma,Jeltema:2008ax}. Constraints on the Milky
Way diffusion parameters can be inferred from
data~\cite{1992ApJ...390...96W,Baltz:1998xv,Maurin:2001sj} and
typically range between $10^{27}$--$10^{29}\, {\rm cm}^2/{\rm s}$.
Similarly, the parameter $\gamma_D$ is expected to lie in the range
$0\leq \gamma_D \leq 1$ \cite{Jeltema:2008ax}.
To be specific, we choose values close to the geometric means of the
individual ranges, namely 
 $D_0 = 3 \times 10^{28}\, {\rm cm}^2/{\rm s}$ and $\gamma_D= 0.3$
\cite{McDaniel:2017ppt}, postponing the discussion
of the dependence on the choices until a little later.

For a given DM particle, the synchrotron flux, understandably, depends
on the states to which it pair-annihilates and their subsequent
cascades. As in the preceding sections, we consider three annihilation
channel states, {\em i.e.}, $b\bar{b}$, $\tau^+ \tau^-$ and
$\mu^+ \mu^-$, and for the sake of simplicity, continue to assume that
a single channel dominates overwhelmingly.  We use the RX-DMFIT
code \cite{McDaniel:2017ppt} for the calculation of synchrotron
flux; to understand the profile, we use a
typical value for the velocity averaged DM annihilation cross section, namely,
$\langle \sigma v \rangle = 10^{-26} \, {\rm cm}^3/{\rm
s}$, postponing a derivation of constraints on the same until
later. For all the dSphs we have used a thermal electron density
$n \approx 10^{-6}$
cm$^{-3}$ \cite{Colafrancesco:2006he,McDaniel:2017ppt},
and the NFW density profile for the DM distribution within.


\begin{figure}[!h]
\centering
  \subfigure[]
    % \centering
  {\includegraphics[width=0.5\linewidth]{figures/dnde_200GeV_r_1e-1kpc_Tucana_II.pdf}}
    %\caption{}
    \label{fig:dnde_200GeV}
  %\end{subfigure}
%\hfill
  \subfigure[]
    % \centering
  {\includegraphics[width=0.5\linewidth]{figures/dnde_2TeV_r_1e-1kpc_Tucana_II.pdf}}
    %\caption{}
    \label{fig:dnde_2TeV}
  %\end{subfigure}
\caption{Solution of the diffusion equation at a radial distance $r=0.1$~kpc 
for Tucana II for three different exclusive annihilation channels, to
  $b\bar{b}$ (red), to $\tau^+ \tau^-$ (green) and to
  $\mu^+ \mu^-$ (blue). Two different DM mass values have been
  considerd, (a) 200 GeV and (b) 2 TeV. For both cases $B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s, $\gamma_D = 0.3$ 
  and $\langle \sigma v\rangle \, = 10^{-26}$ cm$^3$/s have been used.
  NFW density profile has been used for DM distribution inside the dSph. } 
  \label{figure:dnde}
\end{figure}

 Fig.\ref{figure:dnde} shows the stationary electron distribution
spectrum for Tucana II at a radial distance 0.1 kpc for two different
DM mass values, 200 GeV and 2 TeV. With the cascades from a $b$-decay being
capable of producing more $e^\pm$ than a $\tau$ or a $\mu$ can (the latter, only one), it is understandable that the integrated spectrum is much larger for
the $b\bar b$ channel than it is for the others. This also explains
the relative softness of the three spectra in Fig.\ref{figure:dnde}.


\begin{figure}[!h]
\centering
 \includegraphics[width=.49\linewidth,height=3in]{figures/sync_power_vs_E.pdf}
 \caption{Synchrotron power spectrum for different frequencies with magnetic field 1 $\mu$G.}
 \label{figure:synpower}
 \end{figure}

For a given frequency, the energy corresponding to the peak of the
synchrotron power spectrum contributes significantly to $j_{\rm
synch}(\nu,r)$ in Eqn.\ref{eqn:emissivity}. The power spectrum $P_{\rm
synch}(\nu,E,B)$ for $B= 1$ $\mu$G and for different frequencies in
the range 5 MHz-50 GHz are shown in
Fig.\ref{figure:synpower}. Understandably, for higher frequencies, the
synchrotron power peaks at a higher value of energy. Clearly, for a
given frequency, the channel resulting in a larger number of $e^\pm$
with energies closer to the peak of the synchrotron power spectrum
will result in a larger synchrotron flux. Hence, for higher
frequencies, the synchrotron flux from a leptonic channel will
dominate over that from a hadronic channel. This feature can be
observed in Fig.\ref{figure:bbbartautau_flux_comp}, where for a given
DM mass ({\em e.g.}, 200 GeV) the $\tau^+ \tau^-$ channel dominates
over the $b \bar{b}$ channel for higher frequencies; by the same
token, for lower frequencies, the $b\bar{b}$ channel dominates over
the $\tau^+ \tau^-$ channel. Since the electrons originating from the
pair-annihilation of a DM of mass $M_\chi$ can have a maximum energy
$M_\chi$, the spectrum corresponding to a heavier DM would be harder
(as shown by Fig.\ref{figure:dnde}).  Consequently, for larger
frequencies, the synchrotron power spectrum peaks at a higher value of
the electron energy. This is reflected by
Fig.\ref{figure:bbbartautau_flux_comp} where, for a larger $M_\chi$,
the crossover from $b\bar b$ dominance to $\tau^+ \tau^-$ dominance
occurs at progressively higher frequencies.

%%%%%%%
\begin{figure}[h!]
\centering
 \includegraphics[width=.49\linewidth,height=3in]{figures/Tucana_II_bbbar_tautau_mumu_200GeV_2TeV_flux.pdf}
 \caption{Synchrotron flux for three final states for DM annihilation, i.e., 100$\%$ to $b\bar{b}$ (red), 100$\%$ to $\tau^+ \tau^-$ (green) and 100$\%$ $\mu^+ \mu^-$ (blue).
    The solid line corresponds to DM mass 200 GeV and the dashed line corresponds to DM mass 2 TeV. 
    $B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s, $\gamma_D = 0.3$ 
  and $\langle \sigma v\rangle \, = 10^{-26}$ cm$^3$/s have been used.
    NFW density profile has been used for DM distribution inside the dSph. }
 \label{figure:bbbartautau_flux_comp}
 \end{figure}
%%%%%%%%
 

% \subsubsection{Radio limits on $\langle \sigma v \rangle$}

\begin{table}[!h]
\centering
\begin{tabular}{|p{2.5cm}|p{4cm}|p{4cm}|}
\hline \hline
Galaxy &  From GMRT (unit Jy) & From VLA (unit Jy)  \\
& Freqency~=~0.1475 GHz	& Freqency~=~1.4 GHz \\
\hline \hline
Aquarius-II & $3.5 \times10^{-3}$ & $4.4 \times10^{-4}$ \\
\hline \hline
Draco-II & $4.6 \times10^{-3}$ & $5.8 \times10^{-4}$ \\
\hline \hline
Eridanus-II & $4 \times10^{-3}$ & X \\
\hline \hline
Grus-I & $2.1 \times10^{-3}$ & X \\
\hline \hline
Hydra-II & $4.5 \times10^{-3}$ & $5.8 \times10^{-4}$ \\
\hline \hline
Leo-V & $3.1 \times10^{-3}$ & $5 \times10^{-4}$ \\
\hline \hline
Pegasus-III & $5.1 \times10^{-3}$ & $4.9 \times10^{-4}$ \\
\hline \hline
Pisces-II & $1.8 \times10^{-3}$ & $4.5 \times10^{-4}$ \\
\hline \hline
Triangulum-II & $3.1 \times10^{-3}$ & $5.5 \times10^{-4}$ \\
\hline \hline
Draco & $3.7 \times10^{-3}$ & $4.7 \times10^{-4}$ \\
\hline \hline
\end{tabular}
\caption{Upper limits on the radio flux density from the dSphs obtained from GMRT and VLA. The absence of data has been indicated by an ``X''.
For Carina-II, Horologium-II, Reticulum-II and Tucana-II\&III, neither
observatory provides any data.}
\label{table:radio_flux_upper_limits}
\end{table}


%%%%%%
\begin{figure}[h!]
\centering
 \includegraphics[width=.3\linewidth]{figures/bbbar_Exclusion_Curve_GMRT_VLA_comparison_sigmav_versus_M.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/mumu_Exclusion_Curve_GMRT_VLA_comparison_sigmav_versus_M.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/tautau_Exclusion_Curve_GMRT_VLA_comparison_sigmav_versus_M.pdf}

 \hskip 10pt
 \includegraphics[width=0.9\linewidth]{figures/legends_Exclusion.pdf}
\caption{Upper limits on $<\sigma v>$ for different values of DM mass obtained using data from GMRT and VLA. The left, center and right
panels are for $\chi \chi \rightarrow b \bar{b}\ , \ \tau^+ \tau^-\ , \ \mu^+\mu^- $ respectively. 
For each plot $B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s, $\gamma_D = 0.3$ have been used.
NFW density profile has been used for DM distribution inside the dSphs.
For each dSph the values of the parameters $d$, $r_h$, $\rho_s$ and $r_s$  have been used from table \ref{table:astro_param_dwarfs}~. 
}
\label{figure:sigmav_Exclusion_curve}
\end{figure}
%%%%%% 
Of the existing radio-frequency observatories, two particularly
important ones are
\begin{itemize}
\item the Giant Metrewave Radio Telescope (GMRT) \cite{Intema:2016jhx} with its sky-survey, covering the expanse over $-53^{\circ}$ to $+90^{\circ}$, with 
a particularly useful set corresponding to $\nu =0.1475~{\rm GHz}$, and
\item the NVSS survey by the Very Large Array 
(VLA) telescope \cite{condon1998}, over $-40^{\circ}$ to $+90^{\circ}$,
and at $\nu = 1.4~{\rm GHz}$.
\end{itemize}
The non-observation of any emission from the location of the UFDs
under consideration can be tranlsated to 1$\sigma$ level of upper limits on the fluxes same as
listed in Table \ref{table:radio_flux_upper_limits}. Here we would like to mention that all radio interferometric maps are made per unit beam where beam is generally convolved with their respective point spread function (PSF) while making the map. So we can directly obtain the flux density by using the final image in units of Jy. Note here that
the limited sky coverage implies that no statement can be made for
certain UFDs, such as Tucana-II. These limits can, then, be 
translated to upper limits on $\langle
\sigma v \rangle$ for different annihilation channels, as shown in 
Figure \ref{figure:sigmav_Exclusion_curve}. As with the case of the
gamma-ray observations, no such limit can be derived for Hydra II and
Triangulum II as current observations only admit upper limits on their
densities (see Table \ref{table:table-1}).

For a given dSph the upper limit obtained from VLA is stronger
compared to that obtained from GMRT for higher values of DM mass.  The
synchrotron flux for a dSph depends on the choice of magnetic field
(B) and the diffusion coefficient ($D_0$). Hence, the upper limits on
$\langle \sigma v \rangle$ calculated using the upper limit on the
flux will depend on the choice of these parameters.  In
Figure \ref{figure:Exclusion_curve_B_D0_dependence} we show the strong
effect of $B$ and $D_0$ on the resulting upper limit on
$\langle \sigma v\rangle$.  Since Aquarius II gives the strongest
limit on $\langle \sigma v \rangle$ among the newly discovered UFDs,
we choose it to show the effect of $B$ and $D_0$ on the upper limit.
Figure \ref{figure:Exclusion_curve_VLA_Fermilat_comparison} shows the
comparison between the best limits from VLA with the best from
Fermi-LAT for all the three annihilation channels, {\rm i.e.}, $b\bar{b}$, $\mu^+ \mu^-$ and $\tau^+ \tau^-$. For Fermi-LAT
Horologium I gives the best limit and for VLA Draco gives the best
limit among all the considered dSphs. It can be observed that for the mass range 10 GeV-10 TeV VLA gives stronger limit for $\mu^+ \mu^-$ and $\tau^+ \tau^-$, whereas for 
$b\bar{b}$ Fermi-LAT gives stronger constraint towards lower DM mass.


\begin{figure}[h!]
\centering
 \includegraphics[width=.4\linewidth]{figures/Aquarius_II_bbbar_Exclusion_Curve_sigmav_versus_M_B_D0_Dependence.pdf}
 \caption{Upper limits on $\langle \sigma v \rangle$ for $b \bar{b}$ annihilation channel for Aquarius II with different choices of $B$ and $D_0$.
 For all the three cases we have used a constant values for $\gamma_D$ = 0.3.
 NFW density profile has been used for DM distribution inside the dSph.}
 \label{figure:Exclusion_curve_B_D0_dependence}
\end{figure}

%%%%%%
\begin{figure}[h!]
\centering
 \includegraphics[width=.3\linewidth]{figures/bbbar_Exclusion_Curve_sigmav_versus_M_Fermilat_VLA_Comparison.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/mumu_Exclusion_Curve_sigmav_versus_M_Fermilat_VLA_Comparison.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/tautau_Exclusion_Curve_sigmav_versus_M_Fermilat_VLA_Comparison.pdf}
 
 \caption{Comparison of Upper limits on $\langle \sigma v \rangle$ from VLA and Fermi-LAT. We have compared the best limit from VLA (Draco) 
 with the best limit from Fermi-LAT (Horologium I). The left, center and right
panels are for $\chi \chi \rightarrow b \bar{b}\ , \ \tau^+ \tau^-\ \rm{and} \ \mu^+\mu^- $ respectively.
The VLA limit for Draco has been obtained with the astophysical parameters
 $B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s and $\gamma_D = 0.3$. NFW density profile has been used for DM distribution inside the dSph.} 
 \label{figure:Exclusion_curve_VLA_Fermilat_comparison}
\end{figure}


Square Kilometer Array (SKA) is world's largest radio telescope ever
planned and search for particle signature of DM is one of the primary
goals of the project \cite{Bull:2018lat, Colafrancesco:2015ola}.  SKA
will work over a wide radio frequency range 50 MHz - 50 GHz.  This
enables SKA to observe the synchrotron emision from DM annihilation in
astrophysical structures \cite{Bull:2018lat, Colafrancesco:2015ola}.
We calculate the synchrotron flux from the newly discovered dSphs and
study the possibility of observing these signals at SKA.
Fig.\ref{figure:synflux_newgalaxies}, shows the resultant synchrotron
fluxes, for the dSphs listed in Table \ref{table:astro_param_dwarfs},
for each of the three exclusive annhilation channels ($b\bar{b}$,
$\tau^+ \tau^-$ and $\mu^+ \mu^-$). Also shown are the predicted
sensitivity curves for 10 hr, 100 hr and 1000 hr of data collecting
time for the SKA telescope.  The SKA sensitivity limits have been
obtained from \cite{braun2017ska,braun2019anticipated}. For a given
frequency if the synchrotron flux from a dSph lies above the SKA
sensitivity curve then the flux can be observed by the SKA.  We have
calculated the synchrotron flux for two different values of DM mass,
i.e., 200 GeV and 2 TeV.  For the prediction of synchrotron flux we
have used the annihilation cross section $\langle \sigma v \rangle $
$=$ $10^{-26}$ $cm^3/s$.  For both 200 GeV and 2 TeV DM mass
this value of cross section satisfies the upper limits obtained
earlier.


%%%%%%%
\begin{figure}[h!]
\centering
 \includegraphics[width=.3\linewidth]{figures/bbbar_new_udfs_ska_radio_sensitivity_200GeV.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/tautau_new_udfs_ska_radio_sensitivity_200GeV.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/mumu_new_udfs_ska_radio_sensitivity_200GeV.pdf}
 \includegraphics[width=.3\linewidth]{figures/bbbar_new_udfs_ska_radio_sensitivity_2TeV.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/tautau_new_udfs_ska_radio_sensitivity_2TeV.pdf}
\hskip 10pt
 \includegraphics[width=.3\linewidth]{figures/mumu_new_udfs_ska_radio_sensitivity_2TeV.pdf}
 \hskip 10pt
 \includegraphics[width=0.9\linewidth]{figures/legends.pdf}
\caption{Synchrotron fluxes from the new galaxies including Draco. The left, center and right
panels are for $\chi \chi \rightarrow b \bar{b}\ , \ \tau^+ \tau^-\ , \ \mu^+\mu^- $ respectively, while the top (bottom) rows correspond to $M_\chi = 200 \GeV (2 \, {\rm TeV})$. 
For each plot $B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s, $\gamma_D = 0.3$ and $\langle \sigma v\rangle \, = 10^{-26}$ cm$^3$/s have been used.
NFW density profile has been used for DM distribution inside the dSphs. 
For each dSph the values of the parameters $d$, $r_h$, $\rho_s$ and $r_s$  have been used from table \ref{table:astro_param_dwarfs}~. 
}
\label{figure:synflux_newgalaxies}
\end{figure}
%%%%%%



Fig.\ref{figure:synflux_newgalaxies} also contains the synchrotron
flux for one of the well studied classic dSph, namely Draco (with a
$J$-factor of 
$0.679 \times 10^{19}$ GeV$^2$ cm$^{-5}$ at $\theta = 0.5^0$).  It is worth noting
that for an identical choice of parameters $(\langle\sigma v\rangle, B,
D_0, M_{\chi})$, the flux from Draco is expected to be larger than those
from the newly discovered dSphs.
We can observe that a 200 GeV DM annihilating to any one of the three channels $b \bar{b}$, $\mu^+ \mu^-$ and $\tau^+ \tau^-$, 
the synchrotron flux from all the 15 dSphs can be observed with 1000 hrs data collection time at SKA.
For a given annihilation channel if we go higher in DM mass the synchrotron flux decreases and the feasibility of observing radio signals at SKA 
decreases. This can be observed from the plots for 2 TeV DM mass from Figure \ref{figure:synflux_newgalaxies}.
For a 2 TeV DM the synchrotron signals from $b \bar{b}$ channel can be observed at 1000 hr of SKA for all the 15 dSphs. 
But for most of the 15 dSphs the synchrotron signals from $\mu^+ \mu^-$ and $\tau^+ \tau^-$ channels
can not be observed with 1000 hr of data collection time at SKA.
Only for Draco the synchrotron signals for both 200 GeV and 2 TeV DM, and for all the three annihilation channels
can be observed with only 10 hr data of SKA.
 

\begin{figure}[!h]
\centering
  \subfigure[]
     %\centering
 {\includegraphics[width=0.5\linewidth]{figures/Tucana_II_bbbar_200GeV_d_fundamental_uncertainty.pdf}}
    %\caption{}
    \label{fig:d_uncertainty}
  %\end{subfigure}
%\hfill
  \subfigure[]
     %\centering
  {\includegraphics[width=0.5\linewidth]{figures/Tucana_II_bbbar_200GeV_rhalf_fundamental_uncertainty.pdf}}
    %\caption{}
    \label{fig:rhalf_uncertainty}
  %\end{subfigure}
    \subfigure[]
     %\centering
  {\includegraphics[width=0.5\linewidth]{figures/Tucana_II_bbbar_200GeV_sigma_fundamental_uncertainty.pdf}}
   % \caption{}
    \label{fig:sigma_uncertainty}
  %\end{subfigure}
\caption{ Uncertainty in the synchrotron flux from Tucana II due to 1$\sigma$ uncertainty in the parameters (a) $d$, (b) $r_{\frac{1}{2}}$ 
and (c) $\sigma$. NFW density profile has been used for DM distribution inside the dSph. 
We have considered a 200 GeV DM annihilating to $b\bar{b}$ final state. For each of the three cases we have used
$B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s, $\gamma_D = 0.3$ and $\langle \sigma v\rangle \, = 10^{-26}$ cm$^3$/s.
}
   \label{figure:uncertainty}
\end{figure}



\subsection{Uncertainty in Synchrotron flux}
\label{sec:synchrotron_uncertainty}



As with the case for the gamma-ray fluxes, the synchrotron fluxes too
are subject to uncertainties on account of the errors in determining the
the astrophysical parameters $d$, $r_{1/2}$ and $\sigma$. Using the
$1\sigma$ uncertainties
in these, as listed in 
Table \ref{table:astro_fundamental_param_dwarfs}, we show, in
Figure \ref{figure:uncertainty}, the consequent
uncertainities in the synchrotron flux for a 200 GeV DM annihilating to $b\bar{b}$ final
state in Tucana II. The particular UFD is chosen to demonstrate this as it is the
one associated with the highest synchrotron flux.

\begin{figure}[h!]
\centering
 \includegraphics[width=.49\linewidth,height=3in]{figures/bbbar_NFW_Burkert_ISO_Tucana_II_200GeV.pdf}
 \caption{Synchrotron flux vs. frequency for Tucana II for different dark matter distribution profiles : NFW, Burkert and ISO.
 We have considered a 200 GeV DM annihilating to $b\bar{b}$ final state. We have used 
 $B \, = \, 1\, \mu$G, $D_0 = 3 \times 10^{28}$ cm$^2$/s, $\gamma_D = 0.3$ and $\langle \sigma v\rangle \, = 10^{-26}$ cm$^3$/s.}
 \label{figure:sync_profile_dependence}
 \end{figure}

A further source of uncertainty is due to the density distribution for the DM.
While we have, until now, used the NFW profile, in
Fig.\ref{figure:sync_profile_dependence} we display the differences in
predicted flux for Tucana II for NFW, Burkert and ISO profiles. It is
interesting to note that while, for the gamma-ray flux, the NFW
profile closely corresponded to the median prediction, in the present
context it leads to the highest fluxes, while the Burkert profile
leads to the lowest.

The values of magnetic field ($B$), diffusion constant ($D_0$) and the
exponent ($\gamma_D$) for the dSphs are also not known precisely. In
Section \ref{sec:analysis} we discussed about the possible values for
$B$, $D_0$ and $\gamma_D$. To see the effect of these parameters on
the prediction of the amount of synchrotron flux, in
Figure \ref{fig:flux_diff_BD0gamma} we plot the synchrotron flux for
different values of $B$, $D_0$ and $\gamma_D$.  We have taken the
values of $B$ in the range $0.5$-$10$ $\mu$G, $D_0$ in the range
$3\times 10^{26}$-$10^{30}$ $cm^2/s$ and $\gamma_D$ in the range
$0.1$-$1$. Since magnetic field is the cause of synchrotron radiation,
the amount of flux increases as we go higher in magnetic field.  From
Figures \ref{fig:flux_different_D0} and \ref{fig:flux_different_gamma}
we can see how diffusion strongly affects the amount of synchrotron
emission in dSphs \cite{Colafrancesco:2005ji,Colafrancesco:2006he}.





\begin{figure}[!h]
\centering
 \subfigure[]
  %\centering
  {\includegraphics[width=0.5\linewidth]{figures/Tucana_II_bbbar_200GeV_different_B.pdf}}
 % \caption{}
  \label{fig:flux_different_B}
  %\hfill
   \subfigure[]
  %\centering
  {\includegraphics[width=0.5\linewidth]{figures/Tucana_II_bbbar_200GeV_different_D0.pdf}}
  %\caption{}
   \label{fig:flux_different_D0}
  %\end{subfigure}
  %\hfill
   \subfigure[]
  %\centering
  {\includegraphics[width=0.5\linewidth]{figures/Tucana_II_bbbar_200GeV_different_gamma.pdf}}
  %\caption{}
  \label{fig:flux_different_gamma}
  %\end{subfigure}
  \caption{ Synchrotron flux versus frequency for different values of (a) $B$, (b)  $D_0$ and (c) $\gamma_D$.
  The mass of DM is 200 GeV and the DM pair annihilates to $b\bar{b}$ final state with $\langle \sigma v\rangle \, = 10^{-26}$ cm$^3$/s. 
  NFW density profile has been used for DM distribution inside the dSph.}
   \label{fig:flux_diff_BD0gamma}
\end{figure}

\section{Conclusions}\label{section:conclusion}

\noindent Dwarf spheroidal galaxies, apart from being dominated by dark matter,
have almost no millisecond pulsars, and yet possess considerable 
large scale magnetic fields. These render them ideal aren\ae\ for
indirect detection of dark matter through photonic signals.
In this paper, we have studied such signals in two distinct
parts of the electromagnetic spectrum, namely 
high energy gamma rays on the one hand and radio signals on the other.

Eleven years of gamma-ray data collected by the Fermi-LAT
collaboration has failed to show any significant excess from any of
the fifteen ultra faint dwarf spheroidal galaxies. The stringent upper
limits on the $\gamma$-ray flux that these null-results imply are
translated to upper limits on the thermal average of the pair
annihilation cross section $\langle\sigma v\rangle$, for a given value
of $M_{\rm DM}$. We do this for 12 of the UFDs. As for the remaining
three (viz. Triangulum-II, Hydra-II and Tucana-III), since only upper
limits on the corresponding (astrophysical) $J$-factors are available,
the best one can do is to project a {\em best possible} upper bound.

The DM could, of course, annihilate into a plethora of channels, with
the relative probabilities having a strong dependence on the
underlying dynamics governing the system. Rather than be slave to a
particular model, we consider instead that the pair annihilation
proceeds {\em exclusively} through one of three channels, {\em viz.},
$b \bar b$, $\tau^+\tau^- $ and $\mu^+ \mu^-$. The ensuing independent
constraints can, then, be combined to constrain the parameter space of
any model where the annihilation is dominated by one of the three
channels.  Indeed, simple scaling arguments can also be used to infer
bounds applicable for annihilations into other light fermions.

As far as the gamma-ray signal is concerned, of all the dwarf
galaxies, Holorologium-I imposed the most stringent limits, and, for
the $b \bar b$ channel, easily outdoes the limits obtained by the
Planck collaboration.  It needs
to be said here that the limits obtained by us have a significant
dependence on the DM density profile. While most of our results were
derived using the NFW profile, we have considered the Burkert and ISO
profiles as well. In general the Burkert profile led to the strongest
bounds on $\langle \sigma v\rangle$ and the ISO the weakest. Our
limits, thus, represent, typically, the middle-of-the-road
constraints.

On the other hand, electrons produced by the annihilation of
  the dark matter to Standard Model particles emit synchrotron
  radiation as the electrons travel through the magnetic field of the
  dSphs. The synchrotron radiation falls in the radio frequency range.
  We calculated the upper limit on DM annihilation cross section for different annihilation final 
  states, i.e., $b\bar{b}$, $\tau^+ \tau^-$ and $\mu^+ \mu^-$ for the dSphs using the available radio flux upper limits from the GMRT and VLA telescope data. 
  We compared these limits with those obtained from Fermi-LAT data and found that Fermi-LAT gives stongest
  limit. For all dSphs, we have calculated the synchrotron fluxes for
  those aforementioned final states for frequencies ranging from 10 MHz to 100 GHz assuming
  fixed values for annihilation cross section ($\langle \sigma v
  \rangle$), magnetic field $(B)$, diffusion coefficient $(D_0)$ and
  the Kolmogorov parameter ($\gamma_D$).  To showcase the dependence
  of the synchrotron radiation on the dark matter mass we have
  considered two representative values of DM mass, i.e. 200 GeV and 2
  TeV respectively. The SKA telescope will be sensitive between 50 MHz
  to 50 GHz frequency range. We have compared these predicted
  synchrotron flux with the sensitivity curves of SKA telescope for 10
  hr, 100 hr and 1000 hr data collection time.
  

